BioLoom: Scaling Biomedical Vision-Language Models by Learning from the Structure of Scientific Articles

The development of biomedical vision-language models (VLMs) with contrastive image-text pretraining has been driven by scaling to increasingly large and diverse image-text datasets. Beyond scaling, further progress can come from learning richer representations from existing data. We hypothesize that the structure of scientific literature itself provides an additional source of supervision: figures, panels, captions, and accompanying article text encode rich relationships across modalities. Yet, treating these as independent image-text pairs overlooks their relationships. To address this limitation, we incorporate these structural relationships into contrastive image-text supervision. We preserve exact image-text matches while introducing weaker positive supervision for related pairs, such as a panel and the caption of a sibling panel. We upweight cross-article negatives of the same content type to encourage finer discrimination. We also enrich panel descriptions using visual content, original figure captions, and mentioning paragraphs. Pairing panels with these descriptions and whole figures with their original captions yields Loom52M, a dataset of 52.4 million image-text pairs spanning scientific charts and biomedical images. Using Loom52M, BioLoom (DFN-2B) achieves 56.82% domain-balanced mean accuracy across 67 zero-shot classification tasks from 43 datasets in 10 domains, compared with 48.77% for MedPMC-CLIP. On BioLoomBench with concise captions and BioMedFlickr, it achieves bidirectional mean Recall@1 of 63.20% and 10.59%, versus 46.37% and 7.55% for the respective strongest evaluated baselines, BiomedCLIP and MedPMC-CLIP. Code, datasets, benchmarks, and models are available at https://bioloom-clip.github.io/.

==> tables/ablation_pair.tex <==
% Table 6 is inserted later, beside the data-pipeline analysis.
\input{tables/objective_ablation}


==> tables/bioloombench_cap77.tex <==
\ifdefined\jointauccap\begingroup\else\begin{table*}[t]\fi
  \caption{\textbf{Model comparison on BioLoomBench retrieval with original captions and a common 77-token maximum.} Recall@$K$ (\%) is reported in both directions. A model whose native context is shorter than 77 tokens uses its native limit. Biomedical model rows are ordered by bidirectional mean Recall@1 from low to high. Our rows have a light-purple background. I2T and T2I denote image-to-text and text-to-image retrieval, respectively. For \methodname{}, Scratch and DFN-2B denote random and DFN-2B initialization of the vision encoder, respectively; both use the same pretrained text encoder. $^{\ast}$ denotes random vision-encoder initialization for image-text pretraining. Among biomedical models, bold and underlined values indicate the best and second-best scores in each column, respectively.}
  \label{tab:bioloombench-cap77}
  \centering
  \resulttablefont
  \ifdefined\jointauccap\renewcommand{\arraystretch}{1.0}\else\renewcommand{\arraystretch}{1.12}\fi
  \setlength{\tabcolsep}{4pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.22\textwidth}*{6}{Y}}
    \toprule
    & \multicolumn{3}{c}{\textbf{Image $\rightarrow$ Text}} & \multicolumn{3}{c}{\textbf{Text $\rightarrow$ Image}} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    \textbf{Model} & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{18.37} & \tabnum{36.88} & \tabnum{64.68} & \tabnum{18.53} & \tabnum{36.72} & \tabnum{62.48} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{25.34} & \tabnum{47.37} & \tabnum{73.49} & \tabnum{24.68} & \tabnum{45.66} & \tabnum{71.75} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{4.47} & \tabnum{13.69} & \tabnum{30.34} & \tabnum{6.05} & \tabnum{18.04} & \tabnum{37.51} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{19.88} & \tabnum{44.66} & \tabnum{72.75} & \tabnum{9.43} & \tabnum{26.52} & \tabnum{53.27} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{43.39} & \tabnum{72.66} & \tabnum{90.73} & \tabnum{41.75} & \tabnum{70.69} & \tabnum{89.51} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{47.75} & \tabnum{74.83} & \tabnum{91.61} & \tabnum{49.57} & \tabnum{77.01} & \tabnum{92.84} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{50.26} & \tabnum{79.15} & \tabnum{93.98} & \tabnum{48.35} & \tabnum{77.69} & \tabnum{93.53} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{52.09} & \tabnum{78.96} & \tabnum{92.94} & \tabnum{51.89} & \tabnum{78.97} & \tabnum{93.25} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{55.42} & \tabnum{80.70} & \tabnum{93.03} & \tabnum{\underline{56.14}} & \tabnum{\underline{81.63}} & \tabnum{93.35} \\
    \midrule
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{56.03}} & \tabnum{\underline{83.45}} & \tabnum{\underline{95.55}} & \tabnum{53.20} & \tabnum{81.06} & \tabnum{\underline{94.43}} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{63.02}} & \tabnum{\textbf{88.49}} & \tabnum{\textbf{96.73}} & \tabnum{\textbf{61.75}} & \tabnum{\textbf{87.45}} & \tabnum{\textbf{96.61}} \\
    \bottomrule
  \end{tabularx}

\ifdefined\jointauccap\endgroup\else\end{table*}\fi


==> tables/bioloombench_content_r1.tex <==
\begin{table*}[t]
  \caption{\textbf{Model comparison on BioLoomBench retrieval by visual content.} Entries are bidirectional mean Recall@1 (\%), averaging image-to-text (I2T) and text-to-image (T2I) retrieval. The three blocks show concise captions, original captions at native context length, and original captions with a common 77-token maximum. Queries are restricted to each listed content category; the gallery contains all 15,000 figures. Biomedical model rows are ordered by mean Recall@1 across content categories within each caption block. Our rows are shaded light purple. $^{\ast}$ denotes random vision-encoder initialization for image-text pretraining. Among biomedical models, bold and underlined values indicate the best and second-best scores in each column, respectively. Ranks are computed within each caption block.}
  \label{tab:bioloombench-content-r1}
  \centering
  \resulttablefont
  \renewcommand{\arraystretch}{1.12}
  \setlength{\tabcolsep}{5pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.22\textwidth}*{4}{Y}}
    \toprule
    \multicolumn{5}{l}{\textit{Concise caption}} \\
    \textbf{Model} & \textbf{Biological image} & \textbf{Image + chart} & \textbf{Diagram} & \textbf{Chart only} \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{14.86} & \tabnum{16.24} & \tabnum{44.68} & \tabnum{44.53} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{17.65} & \tabnum{20.26} & \tabnum{48.16} & \tabnum{47.43} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{11.47} & \tabnum{1.24} & \tabnum{0.46} & \tabnum{0.57} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{19.79} & \tabnum{12.35} & \tabnum{39.24} & \tabnum{35.60} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{43.73} & \tabnum{32.17} & \tabnum{43.98} & \tabnum{38.93} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{43.54} & \tabnum{32.12} & \tabnum{50.78} & \tabnum{37.23} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{34.78} & \tabnum{32.28} & \tabnum{58.96} & \tabnum{52.77} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{37.85} & \tabnum{35.86} & \tabnum{62.32} & \tabnum{55.10} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{40.77} & \tabnum{42.63} & \tabnum{54.92} & \tabnum{\underline{66.33}} \\
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{55.35}} & \tabnum{\underline{52.95}} & \tabnum{\underline{68.42}} & \tabnum{60.23} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{60.81}} & \tabnum{\textbf{59.38}} & \tabnum{\textbf{72.90}} & \tabnum{\textbf{69.77}} \\
    \midrule
    \multicolumn{5}{l}{\textit{Original caption, native context length}} \\
    \textbf{Model} & \textbf{Biological image} & \textbf{Image + chart} & \textbf{Diagram} & \textbf{Chart only} \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{9.35} & \tabnum{17.12} & \tabnum{35.22} & \tabnum{28.73} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{14.18} & \tabnum{24.97} & \tabnum{43.20} & \tabnum{34.53} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{12.70} & \tabnum{1.32} & \tabnum{0.58} & \tabnum{0.23} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{15.05} & \tabnum{7.78} & \tabnum{25.60} & \tabnum{20.17} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{40.47} & \tabnum{52.65} & \tabnum{59.96} & \tabnum{45.27} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{56.09} & \tabnum{60.99} & \tabnum{53.10} & \tabnum{40.00} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{44.36} & \tabnum{56.00} & \tabnum{62.86} & \tabnum{47.13} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{67.36} & \tabnum{75.12} & \tabnum{65.94} & \tabnum{40.27} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{62.86} & \tabnum{78.27} & \tabnum{67.76} & \tabnum{\textbf{64.13}} \\
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{72.63}} & \tabnum{\underline{84.10}} & \tabnum{\underline{77.64}} & \tabnum{46.60} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{75.45}} & \tabnum{\textbf{85.85}} & \tabnum{\textbf{81.22}} & \tabnum{\underline{61.30}} \\
    \midrule
    \multicolumn{5}{l}{\textit{Original caption, 77-token maximum}} \\
    \textbf{Model} & \textbf{Biological image} & \textbf{Image + chart} & \textbf{Diagram} & \textbf{Chart only} \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{9.35} & \tabnum{17.12} & \tabnum{35.22} & \tabnum{28.73} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{14.18} & \tabnum{24.97} & \tabnum{43.20} & \tabnum{34.53} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{12.70} & \tabnum{1.32} & \tabnum{0.58} & \tabnum{0.23} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{15.05} & \tabnum{7.78} & \tabnum{25.60} & \tabnum{20.17} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{51.32} & \tabnum{32.08} & \tabnum{51.98} & \tabnum{33.30} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{40.47} & \tabnum{52.65} & \tabnum{59.96} & \tabnum{45.27} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{48.25} & \tabnum{45.25} & \tabnum{54.80} & \tabnum{\textbf{58.87}} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{56.09} & \tabnum{\textbf{60.99}} & \tabnum{53.10} & \tabnum{40.00} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{44.36} & \tabnum{56.00} & \tabnum{62.86} & \tabnum{47.13} \\
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{57.48}} & \tabnum{50.74} & \tabnum{\underline{65.32}} & \tabnum{40.50} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{62.52}} & \tabnum{\underline{60.83}} & \tabnum{\textbf{71.20}} & \tabnum{\underline{52.90}} \\
    \bottomrule
  \end{tabularx}

\end{table*}


==> tables/bioloombench_domain_r1.tex <==
\begin{table*}[t]
  \caption{\textbf{Model comparison on BioLoomBench retrieval by domain.} Each entry is bidirectional mean Recall@1 (\%), averaging image-to-text (I2T) and text-to-image (T2I) retrieval. The three blocks use concise captions, original captions at native context length, and original captions with a common 77-token maximum. Short headers follow the 15-domain order listed in Sec.~\ref{app:external-retrieval-benchmark}. Figures from each listed domain are queries; the gallery contains all 15,000 figures. Biomedical model rows are ordered by mean Recall@1 across domains within each caption block. Our rows are shaded light purple. $^{\ast}$ denotes random vision-encoder initialization for image-text pretraining. Within each caption block, bold and underlined values mark the best and second-best biomedical-model scores per column, respectively.}
  \label{tab:bioloombench-domain-r1}
  \centering
  \resulttablefont
  \renewcommand{\arraystretch}{1.12}
  \setlength{\tabcolsep}{1pt}
  \newcommand{\domainheader}{\textbf{Model} & \textbf{Bio} & \textbf{Cell} & \textbf{Cyto} & \textbf{Derm} & \textbf{Dev} & \textbf{Gen} & \textbf{Histo} & \textbf{Micro} & \textbf{Mol} & \textbf{Neuro} & \textbf{Ophth} & \textbf{Phys} & \textbf{Plant} & \textbf{Radio} & \textbf{Surg} \\}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.18\textwidth}*{15}{Y}}
    \toprule
    \multicolumn{16}{l}{\textit{Concise caption}} \\
    \domainheader
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{38.20} & \tabnum{19.90} & \tabnum{14.15} & \tabnum{18.60} & \tabnum{22.15} & \tabnum{32.50} & \tabnum{10.75} & \tabnum{25.00} & \tabnum{19.30} & \tabnum{24.70} & \tabnum{17.75} & \tabnum{32.90} & \tabnum{36.75} & \tabnum{13.10} & \tabnum{23.80} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{40.40} & \tabnum{23.30} & \tabnum{18.20} & \tabnum{18.25} & \tabnum{27.70} & \tabnum{35.85} & \tabnum{14.35} & \tabnum{29.95} & \tabnum{21.55} & \tabnum{29.85} & \tabnum{18.95} & \tabnum{35.75} & \tabnum{40.25} & \tabnum{18.10} & \tabnum{27.60} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{1.40} & \tabnum{1.05} & \tabnum{3.90} & \tabnum{4.80} & \tabnum{6.95} & \tabnum{0.35} & \tabnum{4.75} & \tabnum{1.15} & \tabnum{0.25} & \tabnum{4.50} & \tabnum{5.85} & \tabnum{3.85} & \tabnum{1.80} & \tabnum{25.70} & \tabnum{5.60} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{32.05} & \tabnum{11.35} & \tabnum{9.25} & \tabnum{20.70} & \tabnum{24.10} & \tabnum{23.90} & \tabnum{11.50} & \tabnum{18.55} & \tabnum{15.30} & \tabnum{22.60} & \tabnum{14.15} & \tabnum{32.25} & \tabnum{36.05} & \tabnum{30.15} & \tabnum{26.40} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{41.95} & \tabnum{33.00} & \tabnum{35.45} & \tabnum{42.35} & \tabnum{44.10} & \tabnum{27.30} & \tabnum{36.10} & \tabnum{34.55} & \tabnum{24.00} & \tabnum{46.55} & \tabnum{38.55} & \tabnum{46.00} & \tabnum{31.45} & \tabnum{55.50} & \tabnum{48.95} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{52.55} & \tabnum{35.40} & \tabnum{29.10} & \tabnum{35.80} & \tabnum{40.30} & \tabnum{43.30} & \tabnum{29.55} & \tabnum{41.35} & \tabnum{31.65} & \tabnum{43.85} & \tabnum{33.35} & \tabnum{49.05} & \tabnum{48.35} & \tabnum{39.70} & \tabnum{42.10} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{46.60} & \tabnum{32.55} & \tabnum{34.10} & \tabnum{39.50} & \tabnum{40.90} & \tabnum{34.70} & \tabnum{38.35} & \tabnum{37.30} & \tabnum{28.75} & \tabnum{43.30} & \tabnum{38.20} & \tabnum{43.70} & \tabnum{35.05} & \tabnum{58.55} & \tabnum{47.35} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{55.45} & \tabnum{38.95} & \tabnum{32.60} & \tabnum{37.30} & \tabnum{43.40} & \tabnum{46.05} & \tabnum{33.35} & \tabnum{43.10} & \tabnum{35.50} & \tabnum{47.30} & \tabnum{36.35} & \tabnum{53.05} & \tabnum{51.50} & \tabnum{44.30} & \tabnum{45.65} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{53.85} & \tabnum{41.75} & \tabnum{37.30} & \tabnum{37.75} & \tabnum{42.25} & \tabnum{54.45} & \tabnum{40.20} & \tabnum{50.15} & \tabnum{39.55} & \tabnum{48.80} & \tabnum{40.70} & \tabnum{55.80} & \tabnum{54.10} & \tabnum{53.15} & \tabnum{45.70} \\
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{65.50}} & \tabnum{\underline{57.45}} & \tabnum{\underline{48.85}} & \tabnum{\underline{50.75}} & \tabnum{\underline{56.95}} & \tabnum{\underline{59.55}} & \tabnum{\underline{50.80}} & \tabnum{\underline{60.10}} & \tabnum{\underline{50.40}} & \tabnum{\underline{61.80}} & \tabnum{\underline{49.80}} & \tabnum{\underline{60.80}} & \tabnum{\underline{59.55}} & \tabnum{\underline{65.95}} & \tabnum{\underline{58.75}} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{69.95}} & \tabnum{\textbf{60.45}} & \tabnum{\textbf{55.95}} & \tabnum{\textbf{59.45}} & \tabnum{\textbf{65.95}} & \tabnum{\textbf{65.30}} & \tabnum{\textbf{56.85}} & \tabnum{\textbf{65.50}} & \tabnum{\textbf{54.00}} & \tabnum{\textbf{68.70}} & \tabnum{\textbf{56.05}} & \tabnum{\textbf{67.40}} & \tabnum{\textbf{68.35}} & \tabnum{\textbf{69.45}} & \tabnum{\textbf{64.60}} \\
    \midrule
    \multicolumn{16}{l}{\textit{Original caption, native context length}} \\
    \domainheader
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{31.50} & \tabnum{18.85} & \tabnum{12.15} & \tabnum{12.40} & \tabnum{17.00} & \tabnum{22.65} & \tabnum{11.10} & \tabnum{18.80} & \tabnum{18.10} & \tabnum{20.05} & \tabnum{14.15} & \tabnum{27.45} & \tabnum{27.75} & \tabnum{7.55} & \tabnum{17.25} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{37.45} & \tabnum{27.50} & \tabnum{18.15} & \tabnum{14.50} & \tabnum{24.85} & \tabnum{28.40} & \tabnum{16.30} & \tabnum{26.30} & \tabnum{25.25} & \tabnum{28.30} & \tabnum{19.40} & \tabnum{35.25} & \tabnum{37.05} & \tabnum{13.25} & \tabnum{23.20} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{1.40} & \tabnum{0.75} & \tabnum{4.80} & \tabnum{4.50} & \tabnum{7.35} & \tabnum{0.30} & \tabnum{5.85} & \tabnum{1.30} & \tabnum{0.65} & \tabnum{5.15} & \tabnum{6.55} & \tabnum{4.75} & \tabnum{1.55} & \tabnum{26.75} & \tabnum{7.25} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{22.35} & \tabnum{6.85} & \tabnum{6.75} & \tabnum{13.85} & \tabnum{16.95} & \tabnum{14.40} & \tabnum{7.75} & \tabnum{10.75} & \tabnum{7.05} & \tabnum{14.40} & \tabnum{9.70} & \tabnum{22.55} & \tabnum{24.10} & \tabnum{22.20} & \tabnum{20.15} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{59.35} & \tabnum{52.15} & \tabnum{41.60} & \tabnum{39.20} & \tabnum{52.05} & \tabnum{44.15} & \tabnum{48.30} & \tabnum{47.25} & \tabnum{45.95} & \tabnum{55.25} & \tabnum{42.00} & \tabnum{58.85} & \tabnum{52.60} & \tabnum{44.00} & \tabnum{47.25} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{61.35} & \tabnum{55.70} & \tabnum{45.55} & \tabnum{43.25} & \tabnum{55.80} & \tabnum{46.80} & \tabnum{51.05} & \tabnum{49.65} & \tabnum{48.85} & \tabnum{58.40} & \tabnum{44.40} & \tabnum{63.30} & \tabnum{54.55} & \tabnum{48.70} & \tabnum{52.50} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{57.45} & \tabnum{58.40} & \tabnum{57.25} & \tabnum{52.25} & \tabnum{63.30} & \tabnum{36.00} & \tabnum{65.60} & \tabnum{49.75} & \tabnum{42.20} & \tabnum{64.05} & \tabnum{54.35} & \tabnum{67.15} & \tabnum{45.40} & \tabnum{64.65} & \tabnum{58.90} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{68.90} & \tabnum{68.80} & \tabnum{71.05} & \tabnum{58.35} & \tabnum{76.20} & \tabnum{47.25} & \tabnum{79.85} & \tabnum{60.75} & \tabnum{67.90} & \tabnum{72.55} & \tabnum{66.80} & \tabnum{72.10} & \tabnum{57.75} & \tabnum{76.55} & \tabnum{64.10} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{72.40} & \tabnum{73.30} & \tabnum{69.25} & \tabnum{55.05} & \tabnum{73.50} & \tabnum{\underline{61.35}} & \tabnum{77.25} & \tabnum{67.65} & \tabnum{76.75} & \tabnum{73.80} & \tabnum{65.95} & \tabnum{78.40} & \tabnum{67.90} & \tabnum{69.35} & \tabnum{59.95} \\
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{78.15}} & \tabnum{\underline{79.70}} & \tabnum{\underline{77.20}} & \tabnum{\underline{64.80}} & \tabnum{\underline{82.05}} & \tabnum{59.95} & \tabnum{\underline{83.40}} & \tabnum{\underline{72.15}} & \tabnum{\underline{84.05}} & \tabnum{\underline{79.25}} & \tabnum{\underline{73.05}} & \tabnum{\underline{78.50}} & \tabnum{\underline{68.30}} & \tabnum{\underline{77.90}} & \tabnum{\underline{67.55}} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{82.05}} & \tabnum{\textbf{82.15}} & \tabnum{\textbf{79.45}} & \tabnum{\textbf{69.50}} & \tabnum{\textbf{83.70}} & \tabnum{\textbf{67.25}} & \tabnum{\textbf{84.90}} & \tabnum{\textbf{75.70}} & \tabnum{\textbf{85.00}} & \tabnum{\textbf{83.45}} & \tabnum{\textbf{76.35}} & \tabnum{\textbf{85.25}} & \tabnum{\textbf{74.15}} & \tabnum{\textbf{80.50}} & \tabnum{\textbf{72.80}} \\
    \midrule
    \multicolumn{16}{l}{\textit{Original caption, 77-token maximum}} \\
    \domainheader
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{31.50} & \tabnum{18.85} & \tabnum{12.15} & \tabnum{12.40} & \tabnum{17.00} & \tabnum{22.65} & \tabnum{11.10} & \tabnum{18.80} & \tabnum{18.10} & \tabnum{20.05} & \tabnum{14.15} & \tabnum{27.45} & \tabnum{27.75} & \tabnum{7.55} & \tabnum{17.25} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{37.45} & \tabnum{27.50} & \tabnum{18.15} & \tabnum{14.50} & \tabnum{24.85} & \tabnum{28.40} & \tabnum{16.30} & \tabnum{26.30} & \tabnum{25.25} & \tabnum{28.30} & \tabnum{19.40} & \tabnum{35.25} & \tabnum{37.05} & \tabnum{13.25} & \tabnum{23.20} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{1.40} & \tabnum{0.75} & \tabnum{4.80} & \tabnum{4.50} & \tabnum{7.35} & \tabnum{0.30} & \tabnum{5.85} & \tabnum{1.30} & \tabnum{0.65} & \tabnum{5.15} & \tabnum{6.55} & \tabnum{4.75} & \tabnum{1.55} & \tabnum{26.75} & \tabnum{7.25} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{22.35} & \tabnum{6.85} & \tabnum{6.75} & \tabnum{13.85} & \tabnum{16.95} & \tabnum{14.40} & \tabnum{7.75} & \tabnum{10.75} & \tabnum{7.05} & \tabnum{14.40} & \tabnum{9.70} & \tabnum{22.55} & \tabnum{24.10} & \tabnum{22.20} & \tabnum{20.15} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{46.70} & \tabnum{32.00} & \tabnum{38.70} & \tabnum{45.00} & \tabnum{42.60} & \tabnum{32.50} & \tabnum{48.70} & \tabnum{31.55} & \tabnum{28.25} & \tabnum{44.80} & \tabnum{44.75} & \tabnum{48.45} & \tabnum{35.25} & \tabnum{65.45} & \tabnum{53.90} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{59.35} & \tabnum{52.15} & \tabnum{41.60} & \tabnum{39.20} & \tabnum{52.05} & \tabnum{44.15} & \tabnum{48.30} & \tabnum{47.25} & \tabnum{45.95} & \tabnum{55.25} & \tabnum{42.00} & \tabnum{58.85} & \tabnum{52.60} & \tabnum{44.00} & \tabnum{47.25} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{53.35} & \tabnum{46.20} & \tabnum{44.55} & \tabnum{43.10} & \tabnum{48.25} & \tabnum{\underline{48.70}} & \tabnum{51.15} & \tabnum{44.85} & \tabnum{41.30} & \tabnum{49.85} & \tabnum{46.60} & \tabnum{61.95} & \tabnum{50.80} & \tabnum{59.05} & \tabnum{49.85} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{\underline{61.35}} & \tabnum{55.70} & \tabnum{45.55} & \tabnum{43.25} & \tabnum{55.80} & \tabnum{46.80} & \tabnum{51.05} & \tabnum{49.65} & \tabnum{48.85} & \tabnum{58.40} & \tabnum{44.40} & \tabnum{63.30} & \tabnum{\underline{54.55}} & \tabnum{48.70} & \tabnum{52.50} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{57.45} & \tabnum{\underline{58.40}} & \tabnum{\underline{57.25}} & \tabnum{\underline{52.25}} & \tabnum{\underline{63.30}} & \tabnum{36.00} & \tabnum{\textbf{65.60}} & \tabnum{\underline{49.75}} & \tabnum{42.20} & \tabnum{\underline{64.05}} & \tabnum{\underline{54.35}} & \tabnum{\underline{67.15}} & \tabnum{45.40} & \tabnum{64.65} & \tabnum{\underline{58.90}} \\
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{59.30} & \tabnum{52.65} & \tabnum{52.00} & \tabnum{51.50} & \tabnum{57.20} & \tabnum{47.35} & \tabnum{57.25} & \tabnum{48.55} & \tabnum{\underline{49.20}} & \tabnum{56.55} & \tabnum{53.50} & \tabnum{60.75} & \tabnum{49.85} & \tabnum{\underline{67.10}} & \tabnum{56.50} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{66.35}} & \tabnum{\textbf{61.25}} & \tabnum{\textbf{60.20}} & \tabnum{\textbf{59.30}} & \tabnum{\textbf{65.45}} & \tabnum{\textbf{55.00}} & \tabnum{\underline{65.05}} & \tabnum{\textbf{57.10}} & \tabnum{\textbf{57.10}} & \tabnum{\textbf{65.00}} & \tabnum{\textbf{58.80}} & \tabnum{\textbf{71.90}} & \tabnum{\textbf{59.25}} & \tabnum{\textbf{70.05}} & \tabnum{\textbf{63.95}} \\
    \bottomrule
  \end{tabularx}

\end{table*}


==> tables/bioloombench_retrieval.tex <==
\ifdefined\jointmaintables\begingroup\else\begin{table*}[t]\fi
  \caption{\textbf{Model comparison on BioLoomBench retrieval.} We report Recall@$K$ (R@$K$, \%) for concise and original captions. I2T and T2I denote image-to-text and text-to-image retrieval, respectively. The asterisk and score highlighting follow Tab.~\ref{tab:zero-shot}.}
  \vspace{1mm}
  \label{tab:bioloombench-retrieval}
  \centering
  \resulttablefont
  \renewcommand{\arraystretch}{1.05}
  \setlength{\tabcolsep}{2pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.15\textwidth}*{12}{>{\centering\arraybackslash}X}}
    \toprule
    & \multicolumn{6}{c}{\textbf{Concise caption}} & \multicolumn{6}{c}{\textbf{Original caption}} \\
    \cmidrule(lr){2-7}\cmidrule(lr){8-13}
    \textbf{Model} & \multicolumn{3}{c}{\textbf{I2T}} & \multicolumn{3}{c}{\textbf{T2I}} & \multicolumn{3}{c}{\textbf{I2T}} & \multicolumn{3}{c}{\textbf{T2I}} \\
    & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{24.25} & \tabnum{46.37} & \tabnum{74.44} & \tabnum{22.35} & \tabnum{42.85} & \tabnum{71.15} & \tabnum{18.37} & \tabnum{36.88} & \tabnum{64.68} & \tabnum{18.53} & \tabnum{36.72} & \tabnum{62.48} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{27.65} & \tabnum{50.47} & \tabnum{76.93} & \tabnum{25.69} & \tabnum{47.82} & \tabnum{75.24} & \tabnum{25.34} & \tabnum{47.37} & \tabnum{73.49} & \tabnum{24.68} & \tabnum{45.66} & \tabnum{71.75} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{4.75} & \tabnum{14.76} & \tabnum{33.11} & \tabnum{4.84} & \tabnum{15.87} & \tabnum{35.96} & \tabnum{4.47} & \tabnum{13.69} & \tabnum{30.34} & \tabnum{6.05} & \tabnum{18.04} & \tabnum{37.51} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{27.39} & \tabnum{56.07} & \tabnum{82.69} & \tabnum{16.38} & \tabnum{38.63} & \tabnum{67.55} & \tabnum{19.88} & \tabnum{44.66} & \tabnum{72.75} & \tabnum{9.43} & \tabnum{26.52} & \tabnum{53.27} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{41.27} & \tabnum{70.51} & \tabnum{89.33} & \tabnum{36.84} & \tabnum{63.63} & \tabnum{84.71} & \tabnum{55.42} & \tabnum{80.70} & \tabnum{93.03} & \tabnum{56.14} & \tabnum{81.63} & \tabnum{93.35} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{42.43} & \tabnum{71.55} & \tabnum{92.02} & \tabnum{36.96} & \tabnum{64.62} & \tabnum{87.45} & \tabnum{47.75} & \tabnum{74.83} & \tabnum{91.61} & \tabnum{49.57} & \tabnum{77.01} & \tabnum{92.84} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{44.39} & \tabnum{78.15} & \tabnum{95.83} & \tabnum{35.47} & \tabnum{68.14} & \tabnum{90.77} & \tabnum{67.35} & \tabnum{87.45} & \tabnum{95.83} & \tabnum{67.17} & \tabnum{87.65} & \tabnum{95.90} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{47.11} & \tabnum{76.90} & \tabnum{94.85} & \tabnum{38.74} & \tabnum{66.15} & \tabnum{88.41} & \tabnum{52.09} & \tabnum{78.96} & \tabnum{92.94} & \tabnum{51.89} & \tabnum{78.97} & \tabnum{93.25} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{51.65} & \tabnum{84.38} & \tabnum{97.67} & \tabnum{41.09} & \tabnum{75.63} & \tabnum{94.71} & \tabnum{69.80} & \tabnum{89.67} & \tabnum{97.11} & \tabnum{69.11} & \tabnum{89.48} & \tabnum{96.97} \\
    \midrule
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{61.93}} & \tabnum{\underline{90.61}} & \tabnum{\underline{98.79}} & \tabnum{\underline{52.33}} & \tabnum{\underline{83.86}} & \tabnum{\underline{97.44}} & \tabnum{\underline{75.91}} & \tabnum{\underline{92.94}} & \tabnum{\underline{98.09}} & \tabnum{\underline{74.22}} & \tabnum{\underline{91.52}} & \tabnum{\underline{97.43}} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{66.81}} & \tabnum{\textbf{92.81}} & \tabnum{\textbf{99.28}} & \tabnum{\textbf{59.59}} & \tabnum{\textbf{88.81}} & \tabnum{\textbf{98.77}} & \tabnum{\textbf{79.29}} & \tabnum{\textbf{94.57}} & \tabnum{\textbf{98.39}} & \tabnum{\textbf{78.34}} & \tabnum{\textbf{94.10}} & \tabnum{\textbf{98.41}} \\
    \bottomrule
  \end{tabularx}

\ifdefined\jointmaintables\endgroup\else\end{table*}\fi


==> tables/bootstrap_classification.tex <==
\ifdefined\jointbootstrap\begingroup\else\begin{table*}[p]\fi
\centering
\caption{\textbf{Bootstrap intervals for zero-shot classification.} Each cell reports accuracy (\%) on the first line and its 95\% within-task bootstrap confidence interval below. Task composition and aggregation weights remain fixed.}
\label{tab:bootstrap-classification}
\resulttablefont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{}l*{6}{Y}@{}}
\toprule
Model & Cell & Structure & Microscopy & Cytology & Histopath. & Radiology \\
\midrule
CoCa & \shortstack{\tabnum{22.18}\\{}\tabci{21.30}{22.97}} & \shortstack{\tabnum{33.45}\\{}\tabci{31.55}{35.43}} & \shortstack{\tabnum{56.86}\\{}\tabci{53.76}{59.82}} & \shortstack{\tabnum{41.56}\\{}\tabci{40.40}{42.67}} & \shortstack{\tabnum{39.80}\\{}\tabci{38.52}{41.04}} & \shortstack{\tabnum{36.31}\\{}\tabci{35.00}{37.63}} \\
OpenCLIP & \shortstack{\tabnum{24.49}\\{}\tabci{23.54}{25.44}} & \shortstack{\tabnum{44.44}\\{}\tabci{42.40}{46.27}} & \shortstack{\tabnum{59.04}\\{}\tabci{55.95}{61.99}} & \shortstack{\tabnum{10.25}\\{}\tabci{9.57}{10.95}} & \shortstack{\tabnum{41.03}\\{}\tabci{39.77}{42.24}} & \shortstack{\tabnum{64.86}\\{}\tabci{63.17}{66.50}} \\
\midrule
\mbox{PMC-CLIP} & \shortstack{\tabnum{28.16}\\{}\tabci{27.25}{29.06}} & \shortstack{\tabnum{48.95}\\{}\tabci{47.03}{50.90}} & \shortstack{\tabnum{69.20}\\{}\tabci{67.64}{70.52}} & \shortstack{\tabnum{15.16}\\{}\tabci{14.36}{15.95}} & \shortstack{\tabnum{57.30}\\{}\tabci{56.07}{58.47}} & \shortstack{\tabnum{53.91}\\{}\tabci{52.22}{55.71}} \\
MedSigLIP & \shortstack{\tabnum{22.74}\\{}\tabci{21.79}{23.65}} & \shortstack{\tabnum{44.77}\\{}\tabci{42.87}{46.49}} & \shortstack{\tabnum{65.31}\\{}\tabci{64.05}{66.28}} & \shortstack{\tabnum{37.28}\\{}\tabci{36.19}{38.34}} & \shortstack{\tabnum{38.77}\\{}\tabci{37.70}{39.85}} & \shortstack{\tabnum{49.26}\\{}\tabci{47.56}{51.08}} \\
BiomedCLIP & \shortstack{\tabnum{24.11}\\{}\tabci{23.20}{24.99}} & \shortstack{\tabnum{49.59}\\{}\tabci{47.50}{51.54}} & \shortstack{\tabnum{74.55}\\{}\tabci{73.56}{75.34}} & \shortstack{\tabnum{11.16}\\{}\tabci{10.45}{11.91}} & \shortstack{\tabnum{53.02}\\{}\tabci{51.80}{54.33}} & \shortstack{\tabnum{55.36}\\{}\tabci{53.62}{57.08}} \\
    Panel2Patch & \shortstack{\tabnum{29.40}\\{}\tabci{28.39}{30.40}} & \shortstack{\tabnum{47.12}\\{}\tabci{45.16}{49.07}} & \shortstack{\tabnum{75.66}\\{}\tabci{74.51}{76.54}} & \shortstack{\tabnum{9.50}\\{}\tabci{8.85}{10.18}} & \shortstack{\tabnum{52.30}\\{}\tabci{51.03}{53.70}} & \shortstack{\tabnum{63.31}\\{}\tabci{61.65}{64.92}} \\
\mbox{BMC-CLIP-CF} & \shortstack{\tabnum{24.79}\\{}\tabci{23.99}{25.71}} & \shortstack{\tabnum{56.53}\\{}\tabci{54.69}{58.37}} & \shortstack{\tabnum{69.39}\\{}\tabci{67.25}{71.26}} & \shortstack{\tabnum{8.97}\\{}\tabci{8.38}{9.58}} & \shortstack{\tabnum{51.34}\\{}\tabci{50.06}{52.61}} & \shortstack{\tabnum{60.85}\\{}\tabci{59.22}{62.48}} \\
\mbox{BMC-LongCLIP} & \shortstack{\tabnum{25.62}\\{}\tabci{24.70}{26.55}} & \shortstack{\tabnum{51.49}\\{}\tabci{49.55}{53.44}} & \shortstack{\tabnum{76.23}\\{}\tabci{74.95}{77.21}} & \shortstack{\tabnum{35.61}\\{}\tabci{34.68}{36.58}} & \shortstack{\tabnum{53.94}\\{}\tabci{52.65}{55.20}} & \shortstack{\tabnum{60.73}\\{}\tabci{59.21}{62.15}} \\
\mbox{MedPMC-CLIP} & \shortstack{\tabnum{28.60}\\{}\tabci{27.60}{29.71}} & \shortstack{\tabnum{57.60}\\{}\tabci{55.73}{59.50}} & \shortstack{\tabnum{66.17}\\{}\tabci{63.08}{69.04}} & \shortstack{\tabnum{38.18}\\{}\tabci{37.17}{39.26}} & \shortstack{\tabnum{59.49}\\{}\tabci{58.21}{60.78}} & \shortstack{\tabnum{55.57}\\{}\tabci{53.95}{57.09}} \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \shortstack{\tabnum{34.22}\\{}\tabci{33.29}{35.15}} & \shortstack{\tabnum{56.69}\\{}\tabci{54.90}{58.43}} & \shortstack{\tabnum{79.70}\\{}\tabci{79.17}{80.05}} & \shortstack{\tabnum{37.96}\\{}\tabci{36.86}{39.09}} & \shortstack{\tabnum{61.81}\\{}\tabci{60.61}{63.07}} & \shortstack{\tabnum{64.57}\\{}\tabci{62.95}{66.16}} \\
\rowcolor{bioloomlight}
BioLoom (DFN-2B) & \shortstack{\tabnum{31.05}\\{}\tabci{30.13}{32.00}} & \shortstack{\tabnum{59.73}\\{}\tabci{58.15}{61.42}} & \shortstack{\tabnum{76.32}\\{}\tabci{76.16}{76.49}} & \shortstack{\tabnum{45.61}\\{}\tabci{44.61}{46.58}} & \shortstack{\tabnum{62.55}\\{}\tabci{61.24}{63.78}} & \shortstack{\tabnum{61.40}\\{}\tabci{60.07}{62.71}} \\
\midrule
Model & Ophthalm. & Dermatology & Surgery & Microbial & Overall & \\
\midrule
CoCa & \shortstack{\tabnum{50.53}\\{}\tabci{48.75}{52.41}} & \shortstack{\tabnum{17.37}\\{}\tabci{16.41}{18.38}} & \shortstack{\tabnum{23.05}\\{}\tabci{22.63}{23.47}} & \shortstack{\tabnum{31.48}\\{}\tabci{29.75}{33.34}} & \shortstack{\tabnum{35.26}\\{}\tabci{34.76}{35.76}} & \\
OpenCLIP & \shortstack{\tabnum{42.80}\\{}\tabci{41.07}{44.60}} & \shortstack{\tabnum{15.67}\\{}\tabci{14.70}{16.59}} & \shortstack{\tabnum{31.26}\\{}\tabci{30.89}{31.62}} & \shortstack{\tabnum{44.87}\\{}\tabci{43.05}{46.72}} & \shortstack{\tabnum{37.87}\\{}\tabci{37.36}{38.37}} & \\
\midrule
\mbox{PMC-CLIP} & \shortstack{\tabnum{38.74}\\{}\tabci{36.95}{40.43}} & \shortstack{\tabnum{16.34}\\{}\tabci{15.32}{17.30}} & \shortstack{\tabnum{29.09}\\{}\tabci{28.37}{29.81}} & \shortstack{\tabnum{38.16}\\{}\tabci{36.06}{40.21}} & \shortstack{\tabnum{39.50}\\{}\tabci{39.06}{39.98}} & \\
MedSigLIP & \shortstack{\tabnum{49.24}\\{}\tabci{47.45}{51.17}} & \shortstack{\tabnum{20.62}\\{}\tabci{19.66}{21.63}} & \shortstack{\tabnum{19.38}\\{}\tabci{18.81}{20.00}} & \shortstack{\tabnum{58.58}\\{}\tabci{56.62}{60.91}} & \shortstack{\tabnum{40.59}\\{}\tabci{40.14}{41.04}} & \\
BiomedCLIP & \shortstack{\tabnum{38.27}\\{}\tabci{36.38}{39.98}} & \shortstack{\tabnum{30.48}\\{}\tabci{29.29}{31.67}} & \shortstack{\tabnum{41.83}\\{}\tabci{41.08}{42.61}} & \shortstack{\tabnum{43.63}\\{}\tabci{41.83}{45.53}} & \shortstack{\tabnum{42.20}\\{}\tabci{41.75}{42.64}} & \\
    Panel2Patch & \shortstack{\tabnum{47.56}\\{}\tabci{45.62}{49.33}} & \shortstack{\tabnum{43.76}\\{}\tabci{42.70}{44.80}} & \shortstack{\tabnum{37.34}\\{}\tabci{36.57}{38.03}} & \shortstack{\tabnum{27.77}\\{}\tabci{26.17}{29.51}} & \shortstack{\tabnum{43.37}\\{}\tabci{42.97}{43.78}} & \\
\mbox{BMC-CLIP-CF} & \shortstack{\tabnum{46.38}\\{}\tabci{44.52}{48.17}} & \shortstack{\tabnum{43.76}\\{}\tabci{42.64}{44.85}} & \shortstack{\tabnum{41.35}\\{}\tabci{40.56}{42.10}} & \shortstack{\tabnum{32.25}\\{}\tabci{30.68}{33.92}} & \shortstack{\tabnum{43.56}\\{}\tabci{43.10}{44.01}} & \\
\mbox{BMC-LongCLIP} & \shortstack{\tabnum{35.53}\\{}\tabci{33.84}{37.43}} & \shortstack{\tabnum{40.87}\\{}\tabci{39.60}{42.14}} & \shortstack{\tabnum{37.38}\\{}\tabci{36.53}{38.28}} & \shortstack{\tabnum{28.62}\\{}\tabci{26.83}{30.43}} & \shortstack{\tabnum{44.60}\\{}\tabci{44.15}{45.02}} & \\
\mbox{MedPMC-CLIP} & \shortstack{\tabnum{51.40}\\{}\tabci{49.51}{53.07}} & \shortstack{\tabnum{45.49}\\{}\tabci{44.30}{46.62}} & \shortstack{\tabnum{35.11}\\{}\tabci{34.30}{35.93}} & \shortstack{\tabnum{50.11}\\{}\tabci{48.42}{51.89}} & \shortstack{\tabnum{48.77}\\{}\tabci{48.27}{49.29}} & \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \shortstack{\tabnum{56.65}\\{}\tabci{54.70}{58.41}} & \shortstack{\tabnum{38.75}\\{}\tabci{37.53}{39.91}} & \shortstack{\tabnum{52.65}\\{}\tabci{51.85}{53.52}} & \shortstack{\tabnum{45.90}\\{}\tabci{44.16}{47.61}} & \shortstack{\tabnum{52.89}\\{}\tabci{52.47}{53.30}} & \\
\rowcolor{bioloomlight}
BioLoom (DFN-2B) & \shortstack{\tabnum{61.64}\\{}\tabci{59.72}{63.54}} & \shortstack{\tabnum{48.21}\\{}\tabci{46.99}{49.45}} & \shortstack{\tabnum{57.62}\\{}\tabci{56.77}{58.52}} & \shortstack{\tabnum{64.09}\\{}\tabci{62.11}{65.98}} & \shortstack{\tabnum{56.82}\\{}\tabci{56.40}{57.22}} & \\
\bottomrule
\end{tabularx}
\ifdefined\jointbootstrap\endgroup\else\end{table*}\fi


==> tables/bootstrap_concise.tex <==
\begin{table*}[p]
\centering
\caption{\textbf{BioLoomBench concise-caption retrieval with 95\% query-bootstrap confidence intervals.} Each cell gives Recall@$K$ (\%) and its interval. The gallery and relevance rules match the main evaluation.}
\label{tab:bootstrap-concise}
\resulttablefont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{}l*{6}{Y}@{}}
\toprule
 & \multicolumn{3}{c}{Image-to-text} & \multicolumn{3}{c}{Text-to-image} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Model & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 \\
\midrule
CoCa & \shortstack{\tabnum{24.25}\\{}\tabci{23.57}{24.94}} & \shortstack{\tabnum{46.37}\\{}\tabci{45.57}{47.21}} & \shortstack{\tabnum{74.44}\\{}\tabci{73.78}{75.14}} & \shortstack{\tabnum{22.35}\\{}\tabci{21.70}{23.02}} & \shortstack{\tabnum{42.85}\\{}\tabci{42.00}{43.62}} & \shortstack{\tabnum{71.15}\\{}\tabci{70.43}{71.92}} \\
OpenCLIP & \shortstack{\tabnum{27.65}\\{}\tabci{26.97}{28.35}} & \shortstack{\tabnum{50.47}\\{}\tabci{49.65}{51.27}} & \shortstack{\tabnum{76.93}\\{}\tabci{76.23}{77.57}} & \shortstack{\tabnum{25.69}\\{}\tabci{24.97}{26.38}} & \shortstack{\tabnum{47.82}\\{}\tabci{47.07}{48.60}} & \shortstack{\tabnum{75.24}\\{}\tabci{74.55}{75.90}} \\
\midrule
\mbox{PMC-CLIP} & \shortstack{\tabnum{4.75}\\{}\tabci{4.43}{5.11}} & \shortstack{\tabnum{14.76}\\{}\tabci{14.20}{15.31}} & \shortstack{\tabnum{33.11}\\{}\tabci{32.37}{33.84}} & \shortstack{\tabnum{4.84}\\{}\tabci{4.52}{5.18}} & \shortstack{\tabnum{15.87}\\{}\tabci{15.29}{16.51}} & \shortstack{\tabnum{35.96}\\{}\tabci{35.21}{36.73}} \\
MedSigLIP & \shortstack{\tabnum{27.39}\\{}\tabci{26.70}{28.10}} & \shortstack{\tabnum{56.07}\\{}\tabci{55.31}{56.86}} & \shortstack{\tabnum{82.69}\\{}\tabci{82.12}{83.27}} & \shortstack{\tabnum{16.38}\\{}\tabci{15.81}{16.92}} & \shortstack{\tabnum{38.63}\\{}\tabci{37.86}{39.37}} & \shortstack{\tabnum{67.55}\\{}\tabci{66.84}{68.29}} \\
\mbox{MedPMC-CLIP} & \shortstack{\tabnum{41.27}\\{}\tabci{40.49}{42.05}} & \shortstack{\tabnum{70.51}\\{}\tabci{69.69}{71.23}} & \shortstack{\tabnum{89.33}\\{}\tabci{88.87}{89.85}} & \shortstack{\tabnum{36.84}\\{}\tabci{36.06}{37.58}} & \shortstack{\tabnum{63.63}\\{}\tabci{62.89}{64.37}} & \shortstack{\tabnum{84.71}\\{}\tabci{84.14}{85.31}} \\
    Panel2Patch & \shortstack{\tabnum{42.43}\\{}\tabci{41.61}{43.17}} & \shortstack{\tabnum{71.55}\\{}\tabci{70.85}{72.27}} & \shortstack{\tabnum{92.02}\\{}\tabci{91.62}{92.44}} & \shortstack{\tabnum{36.96}\\{}\tabci{36.19}{37.71}} & \shortstack{\tabnum{64.62}\\{}\tabci{63.86}{65.42}} & \shortstack{\tabnum{87.45}\\{}\tabci{86.92}{87.99}} \\
\mbox{BMC-LongCLIP} & \shortstack{\tabnum{44.39}\\{}\tabci{43.53}{45.20}} & \shortstack{\tabnum{78.15}\\{}\tabci{77.49}{78.81}} & \shortstack{\tabnum{95.83}\\{}\tabci{95.49}{96.14}} & \shortstack{\tabnum{35.47}\\{}\tabci{34.71}{36.25}} & \shortstack{\tabnum{68.14}\\{}\tabci{67.41}{68.90}} & \shortstack{\tabnum{90.77}\\{}\tabci{90.31}{91.25}} \\
\mbox{BMC-CLIP-CF} & \shortstack{\tabnum{47.11}\\{}\tabci{46.33}{47.85}} & \shortstack{\tabnum{76.90}\\{}\tabci{76.21}{77.53}} & \shortstack{\tabnum{94.85}\\{}\tabci{94.47}{95.19}} & \shortstack{\tabnum{38.74}\\{}\tabci{37.91}{39.46}} & \shortstack{\tabnum{66.15}\\{}\tabci{65.39}{66.83}} & \shortstack{\tabnum{88.41}\\{}\tabci{87.92}{88.90}} \\
BiomedCLIP & \shortstack{\tabnum{51.65}\\{}\tabci{50.91}{52.47}} & \shortstack{\tabnum{84.38}\\{}\tabci{83.79}{84.98}} & \shortstack{\tabnum{97.67}\\{}\tabci{97.43}{97.91}} & \shortstack{\tabnum{41.09}\\{}\tabci{40.27}{41.84}} & \shortstack{\tabnum{75.63}\\{}\tabci{74.96}{76.27}} & \shortstack{\tabnum{94.71}\\{}\tabci{94.37}{95.09}} \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \shortstack{\tabnum{61.93}\\{}\tabci{61.20}{62.68}} & \shortstack{\tabnum{90.61}\\{}\tabci{90.14}{91.08}} & \shortstack{\tabnum{98.79}\\{}\tabci{98.61}{98.96}} & \shortstack{\tabnum{52.33}\\{}\tabci{51.53}{53.17}} & \shortstack{\tabnum{83.86}\\{}\tabci{83.29}{84.46}} & \shortstack{\tabnum{97.44}\\{}\tabci{97.18}{97.71}} \\
\rowcolor{bioloomlight}
BioLoom (DFN-2B) & \shortstack{\tabnum{66.81}\\{}\tabci{66.03}{67.54}} & \shortstack{\tabnum{92.81}\\{}\tabci{92.41}{93.22}} & \shortstack{\tabnum{99.28}\\{}\tabci{99.15}{99.41}} & \shortstack{\tabnum{59.59}\\{}\tabci{58.85}{60.35}} & \shortstack{\tabnum{88.81}\\{}\tabci{88.37}{89.31}} & \shortstack{\tabnum{98.77}\\{}\tabci{98.59}{98.94}} \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables/bootstrap_flickr.tex <==
\begin{table*}[p]
\centering
\caption{\textbf{BioMedFlickr retrieval with 95\% query-bootstrap confidence intervals.} Each cell gives Recall@$K$ (\%) and its interval. The gallery and relevance rules match the main evaluation.}
\label{tab:bootstrap-flickr}
\resulttablefont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{}l*{6}{Y}@{}}
\toprule
 & \multicolumn{3}{c}{Image-to-text} & \multicolumn{3}{c}{Text-to-image} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Model & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 \\
\midrule
CoCa & \shortstack{\tabnum{1.64}\\{}\tabci{1.38}{1.93}} & \shortstack{\tabnum{5.58}\\{}\tabci{5.02}{6.11}} & \shortstack{\tabnum{15.30}\\{}\tabci{14.42}{16.10}} & \shortstack{\tabnum{2.06}\\{}\tabci{1.77}{2.38}} & \shortstack{\tabnum{7.95}\\{}\tabci{7.35}{8.60}} & \shortstack{\tabnum{23.98}\\{}\tabci{23.08}{24.96}} \\
OpenCLIP & \shortstack{\tabnum{2.41}\\{}\tabci{2.07}{2.76}} & \shortstack{\tabnum{8.48}\\{}\tabci{7.86}{9.12}} & \shortstack{\tabnum{23.42}\\{}\tabci{22.46}{24.40}} & \shortstack{\tabnum{3.13}\\{}\tabci{2.71}{3.54}} & \shortstack{\tabnum{11.36}\\{}\tabci{10.66}{12.04}} & \shortstack{\tabnum{34.25}\\{}\tabci{33.21}{35.39}} \\
\midrule
\mbox{PMC-CLIP} & \shortstack{\tabnum{2.03}\\{}\tabci{1.71}{2.37}} & \shortstack{\tabnum{8.38}\\{}\tabci{7.75}{9.03}} & \shortstack{\tabnum{25.61}\\{}\tabci{24.63}{26.62}} & \shortstack{\tabnum{2.67}\\{}\tabci{2.31}{3.02}} & \shortstack{\tabnum{11.75}\\{}\tabci{11.05}{12.50}} & \shortstack{\tabnum{34.38}\\{}\tabci{33.26}{35.48}} \\
MedSigLIP & \shortstack{\tabnum{3.56}\\{}\tabci{3.15}{3.98}} & \shortstack{\tabnum{10.83}\\{}\tabci{10.13}{11.55}} & \shortstack{\tabnum{31.45}\\{}\tabci{30.47}{32.51}} & \shortstack{\tabnum{4.62}\\{}\tabci{4.16}{5.08}} & \shortstack{\tabnum{15.18}\\{}\tabci{14.29}{15.99}} & \shortstack{\tabnum{38.78}\\{}\tabci{37.68}{39.87}} \\
BiomedCLIP & \shortstack{\tabnum{4.76}\\{}\tabci{4.27}{5.28}} & \shortstack{\tabnum{14.04}\\{}\tabci{13.26}{14.92}} & \shortstack{\tabnum{35.46}\\{}\tabci{34.43}{36.48}} & \shortstack{\tabnum{4.68}\\{}\tabci{4.22}{5.14}} & \shortstack{\tabnum{19.05}\\{}\tabci{18.18}{19.93}} & \shortstack{\tabnum{50.45}\\{}\tabci{49.23}{51.59}} \\
    Panel2Patch & \shortstack{\tabnum{3.60}\\{}\tabci{3.19}{4.06}} & \shortstack{\tabnum{12.40}\\{}\tabci{11.64}{13.12}} & \shortstack{\tabnum{33.00}\\{}\tabci{31.89}{34.04}} & \shortstack{\tabnum{7.00}\\{}\tabci{6.46}{7.60}} & \shortstack{\tabnum{19.82}\\{}\tabci{18.93}{20.72}} & \shortstack{\tabnum{46.93}\\{}\tabci{45.82}{48.14}} \\
\mbox{BMC-LongCLIP} & \shortstack{\tabnum{5.00}\\{}\tabci{4.50}{5.48}} & \shortstack{\tabnum{15.57}\\{}\tabci{14.75}{16.37}} & \shortstack{\tabnum{37.52}\\{}\tabci{36.40}{38.62}} & \shortstack{\tabnum{6.67}\\{}\tabci{6.08}{7.18}} & \shortstack{\tabnum{20.97}\\{}\tabci{20.01}{21.98}} & \shortstack{\tabnum{52.32}\\{}\tabci{51.11}{53.36}} \\
\mbox{BMC-CLIP-CF} & \shortstack{\tabnum{4.86}\\{}\tabci{4.38}{5.34}} & \shortstack{\tabnum{14.18}\\{}\tabci{13.39}{14.99}} & \shortstack{\tabnum{35.81}\\{}\tabci{34.68}{36.92}} & \shortstack{\tabnum{6.99}\\{}\tabci{6.42}{7.57}} & \shortstack{\tabnum{22.95}\\{}\tabci{22.00}{23.90}} & \shortstack{\tabnum{50.47}\\{}\tabci{49.35}{51.64}} \\
\mbox{MedPMC-CLIP} & \shortstack{\tabnum{5.94}\\{}\tabci{5.39}{6.51}} & \shortstack{\tabnum{19.94}\\{}\tabci{19.04}{20.92}} & \shortstack{\tabnum{45.26}\\{}\tabci{44.13}{46.49}} & \shortstack{\tabnum{9.16}\\{}\tabci{8.50}{9.78}} & \shortstack{\tabnum{31.61}\\{}\tabci{30.51}{32.78}} & \shortstack{\tabnum{61.38}\\{}\tabci{60.28}{62.46}} \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \shortstack{\tabnum{8.00}\\{}\tabci{7.36}{8.60}} & \shortstack{\tabnum{21.85}\\{}\tabci{20.93}{22.83}} & \shortstack{\tabnum{45.66}\\{}\tabci{44.55}{46.92}} & \shortstack{\tabnum{8.84}\\{}\tabci{8.18}{9.52}} & \shortstack{\tabnum{27.63}\\{}\tabci{26.56}{28.70}} & \shortstack{\tabnum{58.75}\\{}\tabci{57.56}{59.92}} \\
\rowcolor{bioloomlight}
BioLoom (DFN-2B) & \shortstack{\tabnum{9.73}\\{}\tabci{8.99}{10.38}} & \shortstack{\tabnum{25.58}\\{}\tabci{24.50}{26.54}} & \shortstack{\tabnum{49.46}\\{}\tabci{48.34}{50.54}} & \shortstack{\tabnum{11.45}\\{}\tabci{10.72}{12.14}} & \shortstack{\tabnum{31.90}\\{}\tabci{30.84}{33.03}} & \shortstack{\tabnum{63.51}\\{}\tabci{62.37}{64.55}} \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables/bootstrap_source.tex <==
\begin{table*}[p]
\centering
\caption{\textbf{BioLoomBench original-caption retrieval with 95\% query-bootstrap confidence intervals.} Each cell gives Recall@$K$ (\%) and its interval. The gallery and relevance rules match the main evaluation.}
\label{tab:bootstrap-source}
\resulttablefont
\setlength{\tabcolsep}{3pt}
\renewcommand{\arraystretch}{1.15}
\begin{tabularx}{\textwidth}{@{}l*{6}{Y}@{}}
\toprule
 & \multicolumn{3}{c}{Image-to-text} & \multicolumn{3}{c}{Text-to-image} \\
\cmidrule(lr){2-4}\cmidrule(lr){5-7}
Model & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 \\
\midrule
CoCa & \shortstack{\tabnum{18.37}\\{}\tabci{17.77}{18.98}} & \shortstack{\tabnum{36.88}\\{}\tabci{36.13}{37.59}} & \shortstack{\tabnum{64.68}\\{}\tabci{63.95}{65.46}} & \shortstack{\tabnum{18.53}\\{}\tabci{17.94}{19.13}} & \shortstack{\tabnum{36.72}\\{}\tabci{35.93}{37.45}} & \shortstack{\tabnum{62.48}\\{}\tabci{61.72}{63.25}} \\
OpenCLIP & \shortstack{\tabnum{25.34}\\{}\tabci{24.65}{26.01}} & \shortstack{\tabnum{47.37}\\{}\tabci{46.49}{48.17}} & \shortstack{\tabnum{73.49}\\{}\tabci{72.78}{74.23}} & \shortstack{\tabnum{24.68}\\{}\tabci{23.99}{25.33}} & \shortstack{\tabnum{45.66}\\{}\tabci{44.85}{46.41}} & \shortstack{\tabnum{71.75}\\{}\tabci{71.03}{72.49}} \\
\midrule
\mbox{PMC-CLIP} & \shortstack{\tabnum{4.47}\\{}\tabci{4.14}{4.81}} & \shortstack{\tabnum{13.69}\\{}\tabci{13.16}{14.26}} & \shortstack{\tabnum{30.34}\\{}\tabci{29.59}{31.05}} & \shortstack{\tabnum{6.05}\\{}\tabci{5.69}{6.43}} & \shortstack{\tabnum{18.04}\\{}\tabci{17.44}{18.65}} & \shortstack{\tabnum{37.51}\\{}\tabci{36.79}{38.28}} \\
MedSigLIP & \shortstack{\tabnum{19.88}\\{}\tabci{19.23}{20.53}} & \shortstack{\tabnum{44.66}\\{}\tabci{43.87}{45.47}} & \shortstack{\tabnum{72.75}\\{}\tabci{72.05}{73.46}} & \shortstack{\tabnum{9.43}\\{}\tabci{8.97}{9.91}} & \shortstack{\tabnum{26.52}\\{}\tabci{25.79}{27.27}} & \shortstack{\tabnum{53.27}\\{}\tabci{52.46}{54.01}} \\
    Panel2Patch & \shortstack{\tabnum{47.75}\\{}\tabci{46.95}{48.52}} & \shortstack{\tabnum{74.83}\\{}\tabci{74.14}{75.49}} & \shortstack{\tabnum{91.61}\\{}\tabci{91.20}{92.07}} & \shortstack{\tabnum{49.57}\\{}\tabci{48.75}{50.33}} & \shortstack{\tabnum{77.01}\\{}\tabci{76.30}{77.65}} & \shortstack{\tabnum{92.84}\\{}\tabci{92.43}{93.25}} \\
\mbox{BMC-CLIP-CF} & \shortstack{\tabnum{52.09}\\{}\tabci{51.32}{52.88}} & \shortstack{\tabnum{78.96}\\{}\tabci{78.27}{79.60}} & \shortstack{\tabnum{92.94}\\{}\tabci{92.53}{93.36}} & \shortstack{\tabnum{51.89}\\{}\tabci{51.09}{52.71}} & \shortstack{\tabnum{78.97}\\{}\tabci{78.33}{79.62}} & \shortstack{\tabnum{93.25}\\{}\tabci{92.87}{93.65}} \\
\mbox{MedPMC-CLIP} & \shortstack{\tabnum{55.42}\\{}\tabci{54.62}{56.21}} & \shortstack{\tabnum{80.70}\\{}\tabci{80.07}{81.31}} & \shortstack{\tabnum{93.03}\\{}\tabci{92.61}{93.41}} & \shortstack{\tabnum{56.14}\\{}\tabci{55.36}{56.95}} & \shortstack{\tabnum{81.63}\\{}\tabci{81.01}{82.25}} & \shortstack{\tabnum{93.35}\\{}\tabci{92.92}{93.73}} \\
\mbox{BMC-LongCLIP} & \shortstack{\tabnum{67.35}\\{}\tabci{66.57}{68.08}} & \shortstack{\tabnum{87.45}\\{}\tabci{86.91}{87.96}} & \shortstack{\tabnum{95.83}\\{}\tabci{95.52}{96.15}} & \shortstack{\tabnum{67.17}\\{}\tabci{66.37}{67.91}} & \shortstack{\tabnum{87.65}\\{}\tabci{87.15}{88.19}} & \shortstack{\tabnum{95.90}\\{}\tabci{95.58}{96.21}} \\
BiomedCLIP & \shortstack{\tabnum{69.80}\\{}\tabci{69.06}{70.56}} & \shortstack{\tabnum{89.67}\\{}\tabci{89.16}{90.18}} & \shortstack{\tabnum{97.11}\\{}\tabci{96.84}{97.39}} & \shortstack{\tabnum{69.11}\\{}\tabci{68.43}{69.81}} & \shortstack{\tabnum{89.48}\\{}\tabci{88.99}{89.95}} & \shortstack{\tabnum{96.97}\\{}\tabci{96.71}{97.24}} \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \shortstack{\tabnum{75.91}\\{}\tabci{75.25}{76.57}} & \shortstack{\tabnum{92.94}\\{}\tabci{92.55}{93.33}} & \shortstack{\tabnum{98.09}\\{}\tabci{97.87}{98.31}} & \shortstack{\tabnum{74.22}\\{}\tabci{73.54}{74.97}} & \shortstack{\tabnum{91.52}\\{}\tabci{91.11}{92.01}} & \shortstack{\tabnum{97.43}\\{}\tabci{97.19}{97.67}} \\
\rowcolor{bioloomlight}
BioLoom (DFN-2B) & \shortstack{\tabnum{79.29}\\{}\tabci{78.63}{79.89}} & \shortstack{\tabnum{94.57}\\{}\tabci{94.24}{94.95}} & \shortstack{\tabnum{98.39}\\{}\tabci{98.17}{98.58}} & \shortstack{\tabnum{78.34}\\{}\tabci{77.68}{79.01}} & \shortstack{\tabnum{94.10}\\{}\tabci{93.73}{94.47}} & \shortstack{\tabnum{98.41}\\{}\tabci{98.21}{98.61}} \\
\bottomrule
\end{tabularx}
\end{table*}


==> tables/data_pipeline_ablation.tex <==
\ifdefined\jointablationtables\begingroup\else\begin{table}[!t]\fi
  \centering
  \caption{\textbf{Ablations of the data pipeline.} We report zero-shot classification accuracy and bidirectional mean R@1 (\%); BioLoomBench uses concise captions. \textit{w/o all charts} removes chart panels and chart-containing whole figures, retaining non-chart panels. \textit{w/ pure-chart views} replaces part of the 25M mixture with figures composed entirely of charts and their panels.}
  \vspace{-1mm}
  \label{tab:ablation}
  \resulttablefont
  \setlength{\tabcolsep}{1.9pt}
  \renewcommand{\arraystretch}{1.12}
  \begin{tabularx}{\columnwidth}{@{}>{\raggedright\arraybackslash}Xccc@{}}
    \toprule
    \textbf{Variant} & \shortstack{\textbf{Zero-shot}\\Mean Acc.} & \shortstack{\textbf{BioLoomBench}\\Mean R@1} & \shortstack{\textbf{BioMedFlickr}\\Mean R@1} \\
    \midrule
    BioLoom (25M pairs) & \tabnum{49.42} & \tabnum{47.73} & \tabnum{6.14} \\
    \midrule
    \rowcolor{ablationcaption}[0pt][0pt]
    \multicolumn{4}{@{}l}{\textit{(a) Caption content}} \\
    Visual description only & \tabnum{49.30} & \tabnum{41.14} & \tabnum{5.81} \\
    Contextual caption only & \tabnum{49.41} & \tabnum{43.76} & \tabnum{6.08} \\
    \midrule
    \rowcolor{ablationviews}[0pt][0pt]
    \multicolumn{4}{@{}l}{\textit{(b) Image views}} \\
    Panel only & \tabnum{40.22} & \tabnum{31.14} & \tabnum{2.57} \\
    Whole figure only & \tabnum{32.49} & \tabnum{15.61} & \tabnum{1.54} \\
    \midrule
    \rowcolor{ablationcharts}[0pt][0pt]
    \multicolumn{4}{@{}l}{\textit{(c) Chart inclusion}} \\
    \mbox{w/o all charts} & \tabnum{47.59} & \tabnum{37.99} & \tabnum{5.83} \\
% Pure-chart views comprise pure-chart whole figures and their constituent panels.
    \mbox{w/ pure-chart views} & \tabnum{44.63} & \tabnum{45.13} & \tabnum{4.57} \\
    \bottomrule
  \end{tabularx}
  \vspace{-2mm}
\ifdefined\jointablationtables\endgroup\else\end{table}\fi


==> tables/dataset_comparison.tex <==
\begin{table}[!t]
  \caption{\textbf{Comparison of biomedical image-text datasets.} Whole/Panel: whole-figure/panel-text pairs; Ctx.: article mentioning paragraphs; Visual: independent image-content descriptions; Bio/Charts: biomedical images and charts/diagrams. $\checkmark$: provided; $\triangle$: subset; $\times$: not specified.}
  \label{tab:dataset-comparison}
  \centering
  \resulttablefont
  \setlength{\tabcolsep}{1pt}
  \renewcommand{\arraystretch}{1.12}
  \begin{tabularx}{\linewidth}{lc>{\hsize=1.2\hsize\linewidth=\hsize\centering\arraybackslash}X>{\hsize=1.0\hsize\linewidth=\hsize\centering\arraybackslash}X>{\hsize=0.75\hsize\linewidth=\hsize\centering\arraybackslash}X>{\hsize=1.15\hsize\linewidth=\hsize\centering\arraybackslash}X>{\hsize=0.65\hsize\linewidth=\hsize\centering\arraybackslash}X>{\hsize=1.25\hsize\linewidth=\hsize\centering\arraybackslash}X}
    \toprule
    & & \multicolumn{2}{c}{\textbf{Views}} & \multicolumn{2}{c}{\textbf{Text}} & \multicolumn{2}{c}{\textbf{Coverage}} \\
    \cmidrule(lr){3-4}\cmidrule(lr){5-6}\cmidrule(lr){7-8}
    \textbf{Dataset} & \textbf{Pairs} & \textbf{Whole} & \textbf{Panel} & \textbf{Ctx.} & \textbf{Visual} & \textbf{Bio} & \textbf{Charts} \\
    \midrule
    ROCO~\cite{pelka2018roco} & 81K & $\checkmark$ & $\times$ & $\times$ & $\times$ & $\checkmark$ & $\times$ \\
    MedICaT~\cite{subramanian2020medicat} & 217K & $\checkmark$ & $\triangle$ & $\triangle$ & $\times$ & $\checkmark$ & $\times$ \\
    PMC-OA~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & 1.65M & $\times$ & $\checkmark$ & $\times$ & $\times$ & $\checkmark$ & $\times$ \\
    PMC-15M~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & 15M & $\checkmark$ & $\times$ & $\times$ & $\times$ & $\checkmark$ & $\checkmark$ \\
    Quilt-1M~\cite{ikezogwo2023quilt} & 1M & $\times$ & $\times$ & $\times$ & $\times$ & $\checkmark$ & $\times$ \\
    BIOMEDICA~\cite{lozano2025biomedica} & 24M & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ & $\checkmark$ & $\checkmark$ \\
    Open-PMC~\cite{baghbanzadeh2025openpmc} & 2.2M & $\times$ & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ \\
    MedPMC~\cite{kim2026medpmc} & 11M & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\times$ & $\checkmark$ & $\times$ \\
    \midrule
    \rowcolor[RGB]{237,244,232}
    Loom52M (Ours) & 52.4M & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $\checkmark$ \\
    \bottomrule
  \end{tabularx}
\end{table}


==> tables/linear_probe_acc.tex <==
\ifdefined\jointlinearprobes\begingroup\else\begin{table*}[t]\fi
\caption{\textbf{Accuracy of linear probes on MedMNIST.} Scores are percentages; column names omit the MNIST suffix. The mean gives equal weight to all 12 datasets. Bold and underlined values indicate the best and second-best scores in each column, respectively.}
\label{tab:linear-probe-acc}
\centering
\resulttablefont
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{1.3pt}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{0.22\textwidth}*{13}{Y}@{}}
\toprule
Model & Path & Chest & Derma & OCT & Pneu. & Blood & Tissue & OrganA & OrganC & OrganS & Retina & Breast & Mean \\
\midrule
CoCa ViT-L/14 & \tabnum{90.36} & \tabnum{94.73} & \tabnum{81.75} & \tabnum{68.80} & \tabnum{83.97} & \tabnum{93.63} & \tabnum{58.87} & \tabnum{87.42} & \tabnum{81.32} & \tabnum{72.84} & \tabnum{60.50} & \tabnum{81.41} & \tabnum{79.63} \\
EVA-CLIP ViT-L/14~\cite{sun2023evaclip} & \tabnum{88.09} & \tabnum{94.74} & \tabnum{80.55} & \tabnum{70.70} & \tabnum{80.45} & \tabnum{94.48} & \tabnum{61.08} & \tabnum{89.13} & \tabnum{83.24} & \tabnum{74.78} & \tabnum{61.50} & \tabnum{82.69} & \tabnum{80.12} \\
RetCCL ResNet-50~\cite{wang2023retccl} & \tabnum{\underline{94.53}} & \tabnum{94.74} & \tabnum{79.15} & \tabnum{58.70} & \tabnum{86.86} & \tabnum{\underline{97.92}} & \tabnum{59.33} & \tabnum{87.27} & \tabnum{84.07} & \tabnum{75.60} & \tabnum{63.25} & \tabnum{83.33} & \tabnum{80.40} \\
SigLIP2 ViT-L/16~\cite{tschannen2025siglip2} & \tabnum{91.85} & \tabnum{94.73} & \tabnum{79.30} & \tabnum{72.10} & \tabnum{88.30} & \tabnum{94.68} & \tabnum{59.63} & \tabnum{90.11} & \tabnum{82.95} & \tabnum{74.06} & \tabnum{61.00} & \tabnum{80.13} & \tabnum{80.74} \\
OpenCLIP (CommonPool) & \tabnum{88.55} & \tabnum{94.73} & \tabnum{82.24} & \tabnum{69.90} & \tabnum{83.01} & \tabnum{95.97} & \tabnum{62.16} & \tabnum{90.43} & \tabnum{84.35} & \tabnum{74.45} & \tabnum{60.75} & \tabnum{86.54} & \tabnum{81.09} \\
ImageNet-1k ResNet-50 & \tabnum{90.46} & \tabnum{94.73} & \tabnum{77.96} & \tabnum{71.20} & \tabnum{86.70} & \tabnum{95.50} & \tabnum{59.50} & \tabnum{91.89} & \tabnum{86.89} & \tabnum{76.12} & \tabnum{60.00} & \tabnum{\underline{87.18}} & \tabnum{81.51} \\
Phikon-v2 ViT-L~\cite{filiot2024phikonv2} & \tabnum{93.80} & \tabnum{94.75} & \tabnum{82.74} & \tabnum{71.10} & \tabnum{87.02} & \tabnum{97.84} & \tabnum{62.27} & \tabnum{87.48} & \tabnum{83.89} & \tabnum{76.27} & \tabnum{59.75} & \tabnum{83.33} & \tabnum{81.69} \\
SigLIP ViT-L/16 & \tabnum{94.32} & \tabnum{94.73} & \tabnum{83.14} & \tabnum{75.30} & \tabnum{87.82} & \tabnum{96.46} & \tabnum{60.85} & \tabnum{90.30} & \tabnum{83.33} & \tabnum{74.25} & \tabnum{61.25} & \tabnum{80.13} & \tabnum{81.82} \\
MetaCLIP ViT-L/14~\cite{xu2024metaclip} & \tabnum{91.87} & \tabnum{94.74} & \tabnum{82.94} & \tabnum{77.80} & \tabnum{87.34} & \tabnum{95.70} & \tabnum{62.29} & \tabnum{88.49} & \tabnum{82.42} & \tabnum{73.60} & \tabnum{62.00} & \tabnum{83.97} & \tabnum{81.93} \\
EVA-02 ViT-L/14~\cite{fang2024eva02} & \tabnum{94.09} & \tabnum{94.75} & \tabnum{80.45} & \tabnum{72.60} & \tabnum{86.06} & \tabnum{96.64} & \tabnum{60.08} & \tabnum{91.26} & \tabnum{88.18} & \tabnum{76.78} & \tabnum{59.50} & \tabnum{84.62} & \tabnum{82.08} \\
CLIP (DFN-2B) ViT-L/14 & \tabnum{92.12} & \tabnum{94.73} & \tabnum{\textbf{84.64}} & \tabnum{72.90} & \tabnum{85.42} & \tabnum{96.29} & \tabnum{61.99} & \tabnum{91.01} & \tabnum{85.55} & \tabnum{74.34} & \tabnum{60.75} & \tabnum{\textbf{89.10}} & \tabnum{82.40} \\
\mbox{PMC-CLIP} ResNet-50 & \tabnum{92.98} & \tabnum{\underline{94.77}} & \tabnum{81.30} & \tabnum{69.50} & \tabnum{\underline{91.35}} & \tabnum{96.84} & \tabnum{\underline{63.51}} & \tabnum{\textbf{92.57}} & \tabnum{\textbf{90.32}} & \tabnum{\underline{77.66}} & \tabnum{62.25} & \tabnum{83.97} & \tabnum{83.09} \\
DINOv2 ViT-L/14~\cite{oquab2024dinov2} & \tabnum{93.62} & \tabnum{94.74} & \tabnum{82.44} & \tabnum{79.50} & \tabnum{87.82} & \tabnum{96.61} & \tabnum{63.33} & \tabnum{90.17} & \tabnum{85.56} & \tabnum{76.79} & \tabnum{\underline{66.50}} & \tabnum{82.69} & \tabnum{83.31} \\
ImageNet-21k ViT-L/16 & \tabnum{93.97} & \tabnum{94.76} & \tabnum{\underline{83.54}} & \tabnum{\underline{79.90}} & \tabnum{87.50} & \tabnum{\textbf{98.22}} & \tabnum{\textbf{64.12}} & \tabnum{\underline{92.30}} & \tabnum{\underline{88.36}} & \tabnum{\textbf{78.14}} & \tabnum{65.00} & \tabnum{\underline{87.18}} & \tabnum{\underline{84.42}} \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \tabnum{\textbf{95.50}} & \tabnum{\textbf{94.83}} & \tabnum{81.50} & \tabnum{\textbf{90.60}} & \tabnum{\textbf{93.75}} & \tabnum{97.11} & \tabnum{59.30} & \tabnum{88.23} & \tabnum{83.63} & \tabnum{75.38} & \tabnum{\textbf{67.00}} & \tabnum{86.54} & \tabnum{\textbf{84.45}} \\
\bottomrule
\end{tabularx}
\ifdefined\jointlinearprobes\endgroup\else\end{table*}\fi


==> tables/linear_probe_auc.tex <==
\ifdefined\jointlinearprobes\begingroup\else\begin{table*}[t]\fi
\caption{\textbf{AUC of linear probes on MedMNIST.} Scores are percentages; column names omit the MNIST suffix. The mean gives equal weight to all 12 datasets. Bold and underlined values indicate the best and second-best scores in each column, respectively.}
\label{tab:linear-probe-auc}
\centering
\resulttablefont
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{1.3pt}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{0.22\textwidth}*{13}{Y}@{}}
\toprule
Model & Path & Chest & Derma & OCT & Pneu. & Blood & Tissue & OrganA & OrganC & OrganS & Retina & Breast & Mean \\
\midrule
CoCa ViT-L/14 & \tabnum{99.23} & \tabnum{66.00} & \tabnum{95.18} & \tabnum{96.48} & \tabnum{96.46} & \tabnum{99.66} & \tabnum{88.34} & \tabnum{99.12} & \tabnum{98.24} & \tabnum{96.62} & \tabnum{83.63} & \tabnum{86.93} & \tabnum{92.16} \\
EVA-CLIP ViT-L/14~\cite{sun2023evaclip} & \tabnum{99.23} & \tabnum{65.33} & \tabnum{94.76} & \tabnum{97.03} & \tabnum{95.41} & \tabnum{99.72} & \tabnum{89.53} & \tabnum{99.30} & \tabnum{98.59} & \tabnum{96.94} & \tabnum{83.58} & \tabnum{86.95} & \tabnum{92.20} \\
EVA-02 ViT-L/14~\cite{fang2024eva02} & \tabnum{99.53} & \tabnum{67.80} & \tabnum{95.03} & \tabnum{97.98} & \tabnum{97.15} & \tabnum{99.86} & \tabnum{89.05} & \tabnum{99.53} & \tabnum{99.13} & \tabnum{97.30} & \tabnum{82.07} & \tabnum{86.53} & \tabnum{92.58} \\
RetCCL ResNet-50~\cite{wang2023retccl} & \tabnum{99.57} & \tabnum{70.92} & \tabnum{93.86} & \tabnum{95.00} & \tabnum{96.96} & \tabnum{99.90} & \tabnum{88.59} & \tabnum{98.95} & \tabnum{98.55} & \tabnum{97.02} & \tabnum{83.44} & \tabnum{88.18} & \tabnum{92.58} \\
OpenCLIP (CommonPool) & \tabnum{99.51} & \tabnum{67.77} & \tabnum{96.06} & \tabnum{95.61} & \tabnum{95.86} & \tabnum{99.81} & \tabnum{89.94} & \tabnum{99.43} & \tabnum{98.76} & \tabnum{96.93} & \tabnum{84.55} & \tabnum{89.16} & \tabnum{92.78} \\
SigLIP2 ViT-L/16~\cite{tschannen2025siglip2} & \tabnum{99.29} & \tabnum{72.36} & \tabnum{95.11} & \tabnum{98.06} & \tabnum{97.73} & \tabnum{99.73} & \tabnum{88.72} & \tabnum{99.36} & \tabnum{98.48} & \tabnum{96.74} & \tabnum{83.91} & \tabnum{86.42} & \tabnum{92.99} \\
DINOv2 ViT-L/14~\cite{oquab2024dinov2} & \tabnum{99.36} & \tabnum{62.88} & \tabnum{96.21} & \tabnum{\underline{99.14}} & \tabnum{97.52} & \tabnum{99.86} & \tabnum{\underline{90.74}} & \tabnum{99.35} & \tabnum{98.82} & \tabnum{97.29} & \tabnum{\textbf{88.77}} & \tabnum{88.45} & \tabnum{93.20} \\
MetaCLIP ViT-L/14~\cite{xu2024metaclip} & \tabnum{\underline{99.58}} & \tabnum{69.21} & \tabnum{95.98} & \tabnum{97.77} & \tabnum{97.59} & \tabnum{99.83} & \tabnum{89.90} & \tabnum{99.15} & \tabnum{98.56} & \tabnum{96.85} & \tabnum{84.99} & \tabnum{89.43} & \tabnum{93.24} \\
SigLIP ViT-L/16 & \tabnum{99.44} & \tabnum{73.67} & \tabnum{96.30} & \tabnum{98.47} & \tabnum{97.84} & \tabnum{99.86} & \tabnum{89.22} & \tabnum{99.41} & \tabnum{98.57} & \tabnum{96.88} & \tabnum{84.20} & \tabnum{85.17} & \tabnum{93.25} \\
CLIP (DFN-2B) ViT-L/14 & \tabnum{\underline{99.58}} & \tabnum{69.57} & \tabnum{\textbf{96.87}} & \tabnum{98.41} & \tabnum{97.33} & \tabnum{99.87} & \tabnum{89.97} & \tabnum{99.47} & \tabnum{98.90} & \tabnum{96.96} & \tabnum{84.25} & \tabnum{89.66} & \tabnum{93.40} \\
Phikon-v2 ViT-L~\cite{filiot2024phikonv2} & \tabnum{99.49} & \tabnum{73.45} & \tabnum{96.10} & \tabnum{96.37} & \tabnum{97.93} & \tabnum{\underline{99.91}} & \tabnum{90.16} & \tabnum{99.01} & \tabnum{98.75} & \tabnum{97.23} & \tabnum{82.77} & \tabnum{92.50} & \tabnum{93.64} \\
ImageNet-1k ResNet-50 & \tabnum{99.15} & \tabnum{74.01} & \tabnum{93.51} & \tabnum{98.21} & \tabnum{97.18} & \tabnum{99.81} & \tabnum{88.69} & \tabnum{\underline{99.59}} & \tabnum{99.05} & \tabnum{97.31} & \tabnum{83.99} & \tabnum{\underline{93.25}} & \tabnum{93.65} \\
\mbox{PMC-CLIP} ResNet-50 & \tabnum{99.52} & \tabnum{\underline{76.51}} & \tabnum{95.76} & \tabnum{97.30} & \tabnum{\underline{98.97}} & \tabnum{99.88} & \tabnum{90.62} & \tabnum{99.52} & \tabnum{\textbf{99.37}} & \tabnum{\textbf{97.68}} & \tabnum{84.77} & \tabnum{92.40} & \tabnum{\underline{94.36}} \\
ImageNet-21k ViT-L/16 & \tabnum{99.52} & \tabnum{74.59} & \tabnum{\underline{96.80}} & \tabnum{98.93} & \tabnum{98.01} & \tabnum{\textbf{99.95}} & \tabnum{\textbf{91.12}} & \tabnum{\textbf{99.60}} & \tabnum{\underline{99.21}} & \tabnum{\underline{97.66}} & \tabnum{86.39} & \tabnum{\textbf{94.28}} & \tabnum{\textbf{94.67}} \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \tabnum{\textbf{99.60}} & \tabnum{\textbf{78.05}} & \tabnum{95.79} & \tabnum{\textbf{99.61}} & \tabnum{\textbf{99.27}} & \tabnum{99.86} & \tabnum{88.27} & \tabnum{99.11} & \tabnum{98.64} & \tabnum{97.00} & \tabnum{\underline{87.25}} & \tabnum{87.68} & \tabnum{94.18} \\
\bottomrule
\end{tabularx}
\ifdefined\jointlinearprobes\endgroup\else\end{table*}\fi


==> tables/linear_probe_f1.tex <==
\ifdefined\jointlinearprobes\begingroup\else\begin{table*}[t]\fi
\caption{\textbf{Macro-F1 of linear probes on MedMNIST.} Scores are percentages; column names omit the MNIST suffix. The mean gives equal weight to all 12 datasets. Bold and underlined values indicate the best and second-best scores in each column, respectively.}
\label{tab:linear-probe-f1}
\centering
\resulttablefont
\renewcommand{\arraystretch}{1.0}
\setlength{\tabcolsep}{1.3pt}
\begin{tabularx}{\textwidth}{@{}>{\raggedright\arraybackslash}p{0.22\textwidth}*{13}{Y}@{}}
\toprule
Model & Path & Chest & Derma & OCT & Pneu. & Blood & Tissue & OrganA & OrganC & OrganS & Retina & Breast & Mean \\
\midrule
CoCa ViT-L/14 & \tabnum{87.66} & \tabnum{0.39} & \tabnum{59.74} & \tabnum{64.53} & \tabnum{81.51} & \tabnum{92.82} & \tabnum{45.98} & \tabnum{85.66} & \tabnum{78.48} & \tabnum{66.71} & \tabnum{42.48} & \tabnum{71.16} & \tabnum{64.76} \\
EVA-CLIP ViT-L/14~\cite{sun2023evaclip} & \tabnum{86.44} & \tabnum{0.60} & \tabnum{58.11} & \tabnum{66.40} & \tabnum{76.26} & \tabnum{94.11} & \tabnum{48.94} & \tabnum{88.13} & \tabnum{79.88} & \tabnum{68.97} & \tabnum{42.56} & \tabnum{73.15} & \tabnum{65.30} \\
RetCCL ResNet-50~\cite{wang2023retccl} & \tabnum{\underline{92.86}} & \tabnum{2.20} & \tabnum{53.69} & \tabnum{53.53} & \tabnum{84.83} & \tabnum{\underline{98.02}} & \tabnum{46.19} & \tabnum{85.61} & \tabnum{81.42} & \tabnum{70.07} & \tabnum{43.48} & \tabnum{75.55} & \tabnum{65.62} \\
SigLIP2 ViT-L/16~\cite{tschannen2025siglip2} & \tabnum{89.16} & \tabnum{1.45} & \tabnum{57.00} & \tabnum{67.75} & \tabnum{86.62} & \tabnum{94.08} & \tabnum{47.48} & \tabnum{89.54} & \tabnum{80.39} & \tabnum{68.95} & \tabnum{43.28} & \tabnum{68.41} & \tabnum{66.18} \\
ImageNet-1k ResNet-50 & \tabnum{86.90} & \tabnum{3.59} & \tabnum{54.55} & \tabnum{67.57} & \tabnum{84.67} & \tabnum{95.52} & \tabnum{47.46} & \tabnum{91.05} & \tabnum{85.11} & \tabnum{71.46} & \tabnum{39.58} & \tabnum{81.20} & \tabnum{67.39} \\
SigLIP ViT-L/16 & \tabnum{91.48} & \tabnum{1.77} & \tabnum{67.81} & \tabnum{72.25} & \tabnum{86.06} & \tabnum{95.89} & \tabnum{48.05} & \tabnum{88.71} & \tabnum{80.05} & \tabnum{69.05} & \tabnum{41.82} & \tabnum{67.60} & \tabnum{67.55} \\
OpenCLIP (CommonPool) & \tabnum{86.62} & \tabnum{0.64} & \tabnum{62.41} & \tabnum{68.89} & \tabnum{80.01} & \tabnum{95.63} & \tabnum{50.74} & \tabnum{89.60} & \tabnum{81.68} & \tabnum{68.68} & \tabnum{46.36} & \tabnum{80.04} & \tabnum{67.61} \\
MetaCLIP ViT-L/14~\cite{xu2024metaclip} & \tabnum{90.10} & \tabnum{0.94} & \tabnum{65.43} & \tabnum{75.19} & \tabnum{85.41} & \tabnum{95.32} & \tabnum{50.38} & \tabnum{86.87} & \tabnum{79.43} & \tabnum{67.66} & \tabnum{42.20} & \tabnum{73.87} & \tabnum{67.73} \\
EVA-02 ViT-L/14~\cite{fang2024eva02} & \tabnum{91.63} & \tabnum{1.33} & \tabnum{58.91} & \tabnum{71.00} & \tabnum{83.75} & \tabnum{96.42} & \tabnum{48.23} & \tabnum{90.28} & \tabnum{86.19} & \tabnum{71.38} & \tabnum{44.59} & \tabnum{77.43} & \tabnum{68.43} \\
Phikon-v2 ViT-L~\cite{filiot2024phikonv2} & \tabnum{91.50} & \tabnum{3.15} & \tabnum{63.24} & \tabnum{69.70} & \tabnum{84.96} & \tabnum{97.96} & \tabnum{50.63} & \tabnum{86.45} & \tabnum{81.09} & \tabnum{70.56} & \tabnum{47.71} & \tabnum{76.06} & \tabnum{68.58} \\
CLIP (DFN-2B) ViT-L/14 & \tabnum{89.85} & \tabnum{1.26} & \tabnum{66.64} & \tabnum{71.14} & \tabnum{83.10} & \tabnum{95.97} & \tabnum{50.90} & \tabnum{89.68} & \tabnum{82.88} & \tabnum{68.69} & \tabnum{43.85} & \tabnum{\textbf{84.50}} & \tabnum{69.04} \\
DINOv2 ViT-L/14~\cite{oquab2024dinov2} & \tabnum{91.11} & \tabnum{1.08} & \tabnum{63.58} & \tabnum{78.96} & \tabnum{86.02} & \tabnum{96.64} & \tabnum{\underline{52.36}} & \tabnum{89.59} & \tabnum{83.80} & \tabnum{72.29} & \tabnum{\textbf{52.66}} & \tabnum{73.77} & \tabnum{70.15} \\
\mbox{PMC-CLIP} ResNet-50 & \tabnum{90.27} & \tabnum{\underline{5.06}} & \tabnum{62.40} & \tabnum{66.34} & \tabnum{\underline{90.29}} & \tabnum{96.81} & \tabnum{51.90} & \tabnum{\textbf{92.07}} & \tabnum{\textbf{88.63}} & \tabnum{\underline{72.62}} & \tabnum{49.82} & \tabnum{76.74} & \tabnum{70.25} \\
ImageNet-21k ViT-L/16 & \tabnum{91.35} & \tabnum{3.54} & \tabnum{\textbf{68.91}} & \tabnum{\underline{79.50}} & \tabnum{85.53} & \tabnum{\textbf{98.35}} & \tabnum{\textbf{54.05}} & \tabnum{\underline{91.58}} & \tabnum{\underline{86.86}} & \tabnum{\textbf{73.96}} & \tabnum{\underline{52.01}} & \tabnum{\underline{82.60}} & \tabnum{\textbf{72.36}} \\
\midrule
\rowcolor{bioloomlight}
BioLoom (Scratch) & \tabnum{\textbf{93.49}} & \tabnum{\textbf{8.52}} & \tabnum{\underline{68.24}} & \tabnum{\textbf{90.45}} & \tabnum{\textbf{93.09}} & \tabnum{96.99} & \tabnum{46.86} & \tabnum{86.71} & \tabnum{80.36} & \tabnum{70.47} & \tabnum{50.00} & \tabnum{81.22} & \tabnum{\underline{72.20}} \\
\bottomrule
\end{tabularx}
\ifdefined\jointlinearprobes\endgroup\else\end{table*}\fi


==> tables/objective_ablation.tex <==
\ifdefined\jointablationtables\begingroup\else\begin{table}[t]\fi
  \centering
  \caption{\textbf{Vision initialization and contrastive-objective ablations.} We report zero-shot accuracy and bidirectional mean R@1 (\%); BioLoomBench uses concise captions. Pair sets follow Sec.~\ref{sec:labels}: semi-positive pairs ($\mathcal{P}_i$) are non-exact pairs within a figure; cross-figure pairs ($\mathcal{A}_i$) span different figures in one article.}
  \vspace{-1mm}
  \label{tab:objective-ablation}
  \resulttablefont
  \setlength{\tabcolsep}{1.1pt}
  \renewcommand{\arraystretch}{1.12}
  \begin{tabularx}{\columnwidth}{@{}>{\raggedright\arraybackslash}Xccc@{}}
    \toprule
    \textbf{Variant} & {\fontsize{7.8}{9.5}\selectfont \shortstack{\textbf{Zero-shot}\\Mean Acc.}} & {\fontsize{7.8}{9.5}\selectfont \shortstack{\textbf{BioLoomBench}\\Mean R@1}} & {\fontsize{7.8}{9.5}\selectfont \shortstack{\textbf{BioMedFlickr}\\Mean R@1}} \\
    \midrule
    \rowcolor{ablationinit}[0pt][0pt]
    \multicolumn{4}{@{}l}{\textit{(a) Vision initialization (ViT-L/14)}} \\
    BioLoom (Scratch) & \tabnum{52.89} & \tabnum{57.13} & \tabnum{8.42} \\
    CommonPool & \tabnum{53.66} & \tabnum{61.53} & \tabnum{10.69} \\
    DINOv2~\cite{oquab2024dinov2} & \tabnum{54.94} & \tabnum{61.20} & \tabnum{10.19} \\
    DFN-2B & \tabnum{56.82} & \tabnum{63.20} & \tabnum{10.59} \\
    \midrule
    \rowcolor{ablationobjective}[0pt][0pt]
    \multicolumn{4}{@{}l}{\textit{(b) Contrastive objective (Scratch)}} \\
    Standard InfoNCE & \tabnum{51.55} & \tabnum{49.71} & \tabnum{6.60} \\
    \addlinespace[2pt]
    \rowcolor{ablationobjective!65!white}[0pt][0pt]
    \multicolumn{4}{@{}l}{\textit{Exact-pair alignment with related-pair masking ($\mathcal{L}_{\mathrm{mask}}$)}} \\
    \mbox{w/o semi-positive mask~($\mathcal{P}_i$)} & \tabnum{52.48} & \tabnum{53.91} & \tabnum{7.52} \\
    \mbox{w/o cross-figure mask~($\mathcal{A}_i$)} & \tabnum{53.31} & \tabnum{54.21} & \tabnum{7.34} \\
    \mbox{w/o both masks~($\mathcal{P}_i\cup\mathcal{A}_i$)} & \tabnum{52.19} & \tabnum{52.44} & \tabnum{6.98} \\
    \addlinespace[2pt]
    \rowcolor{ablationobjective!65!white}[0pt][0pt]
    \multicolumn{4}{@{}l}{\textit{Semi-positive alignment ($\mathcal{L}_{\mathrm{rel}}$)}} \\
    w/o relation loss & \tabnum{52.24} & \tabnum{51.68} & \tabnum{7.24} \\
    w/ exact pairs ($\mathcal{E}_i$) & \tabnum{54.41} & \tabnum{52.79} & \tabnum{7.30} \\
    \mbox{w/o cross-figure mask~($\mathcal{A}_i$)} & \tabnum{49.85} & \tabnum{54.53} & \tabnum{7.90} \\
    \mbox{w/o hard-neg. emphasis} & \tabnum{50.71} & \tabnum{55.48} & \tabnum{7.93} \\
    \bottomrule
  \end{tabularx}
\ifdefined\jointablationtables\endgroup\else
  % Keep the following paragraph close to this standalone table.
  \vspace{-10pt}
\end{table}\fi


==> tables/retrieval.tex <==
\ifdefined\jointretrievalplot\else\begin{table}[t]\fi
  \caption{\textbf{Model comparison on BioMedFlickr retrieval.} Recall@$K$ (\%) is reported for 7,185 image-caption pairs under our revised evaluation protocol. R@$K$ denotes Recall@$K$. The asterisk and score highlighting follow Tab.~\ref{tab:zero-shot}.}
  \vspace{-1.5mm}
  \label{tab:retrieval}
  \centering
  \begingroup
  \resulttablefont
  % Retrieval scores fit two integer digits; reserve more space for model names.
  \renewcommand{\tabnum}[1]{\makebox[\widthof{\normalfont 00.00}][r]{#1}}
  \renewcommand{\arraystretch}{1.05}
  \setlength{\tabcolsep}{1.5pt}
  \begin{tabularx}{\linewidth}{@{}>{\raggedright\arraybackslash}Xrrrrrr@{}}
    \toprule
    & \multicolumn{3}{c}{\textbf{Image $\rightarrow$ Text}} & \multicolumn{3}{c}{\textbf{Text $\rightarrow$ Image}} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    \textbf{Model} & \multicolumn{1}{c}{{R@1}} & \multicolumn{1}{c}{{R@10}} & \multicolumn{1}{c}{{R@100}} & \multicolumn{1}{c}{{R@1}} & \multicolumn{1}{c}{{R@10}} & \multicolumn{1}{c}{{R@100}} \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{1.64} & \tabnum{5.58} & \tabnum{15.30} & \tabnum{2.06} & \tabnum{7.95} & \tabnum{23.98} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{2.41} & \tabnum{8.48} & \tabnum{23.42} & \tabnum{3.13} & \tabnum{11.36} & \tabnum{34.25} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{2.03} & \tabnum{8.38} & \tabnum{25.61} & \tabnum{2.67} & \tabnum{11.75} & \tabnum{34.38} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{3.56} & \tabnum{10.83} & \tabnum{31.45} & \tabnum{4.62} & \tabnum{15.18} & \tabnum{38.78} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{4.76} & \tabnum{14.04} & \tabnum{35.46} & \tabnum{4.68} & \tabnum{19.05} & \tabnum{50.45} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{3.60} & \tabnum{12.40} & \tabnum{33.00} & \tabnum{7.00} & \tabnum{19.82} & \tabnum{46.93} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{5.00} & \tabnum{15.57} & \tabnum{37.52} & \tabnum{6.67} & \tabnum{20.97} & \tabnum{52.32} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{4.86} & \tabnum{14.18} & \tabnum{35.81} & \tabnum{6.99} & \tabnum{22.95} & \tabnum{50.47} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{5.94} & \tabnum{19.94} & \tabnum{45.26} & \tabnum{\underline{9.16}} & \tabnum{\underline{31.61}} & \tabnum{\underline{61.38}} \\
    \midrule
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{8.00}} & \tabnum{\underline{21.85}} & \tabnum{\underline{45.66}} & \tabnum{8.84} & \tabnum{27.63} & \tabnum{58.75} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{9.73}} & \tabnum{\textbf{25.58}} & \tabnum{\textbf{49.46}} & \tabnum{\textbf{11.45}} & \tabnum{\textbf{31.90}} & \tabnum{\textbf{63.51}} \\
    \bottomrule
  \end{tabularx}
  \endgroup
\ifdefined\jointretrievalplot\else\end{table}\fi


==> tables/retrieval_linear_probe.tex <==
% Main-evaluation retrieval table and linear-probing figure share one row.
\begin{table*}[!t]
  \def\jointretrievalplot{1}
  \noindent\begin{minipage}[t]{\columnwidth}
    \vspace{0pt}
    \input{tables/retrieval}
  \end{minipage}\hfill
  \begin{minipage}[t]{\columnwidth}
    \vspace{0pt}
    \centering
    \includegraphics[width=\linewidth]{figures/linear_probe_medmnist.pdf}
    \captionsetup{skip=4.5pt,justification=raggedright,singlelinecheck=false}
    \captionof{figure}{\textbf{Linear probing on MedMNIST.} Accuracy and Macro-F1 are averaged equally over 12 datasets. Star: BioLoom; black outlines: biomedical-pretrained models.}%\Ale{maybe put this on the appendix and instead do  Mean Accuracy vs Model Size? Thus you show your model is not only better but also smaller than Deepmind's} %\yuwei{I think maybe we should keep this figure here, model size is not main comparison, the overall structure is the same as BMC-LongCLIP.}
    \label{fig:linear-probe-medmnist}
  \end{minipage}
  \vspace{-2mm}
\end{table*}


==> tables/retrieval_official_exact.tex <==
\ifdefined\jointbootstrap\begingroup\else\begin{table*}[t]\fi
  \caption{\textbf{Model comparison on BioMedFlickr under the original exact-pair protocol.} We report our evaluations of all models; only the paired row is relevant for Recall@$K$ (\%). Biomedical model rows are ordered by bidirectional mean Recall@1 from low to high. Our rows have a light-purple background. I2T and T2I denote image-to-text and text-to-image retrieval, respectively. $^{\ast}$ denotes random vision-encoder initialization for image-text pretraining. Among biomedical models, bold and underlined values indicate the best and second-best scores in each column, respectively.}
  \label{tab:retrieval-official-exact}
  \centering
  \resulttablefont
  \renewcommand{\arraystretch}{1.12}
  \setlength{\tabcolsep}{4pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.22\textwidth}*{6}{Y}}
    \toprule
    & \multicolumn{3}{c}{\textbf{Image $\rightarrow$ Text}} & \multicolumn{3}{c}{\textbf{Text $\rightarrow$ Image}} \\
    \cmidrule(lr){2-4}\cmidrule(lr){5-7}
    \textbf{Model} & R@1 & R@10 & R@100 & R@1 & R@10 & R@100 \\
    \midrule
    Random & \tabnum{0.01} & \tabnum{0.14} & \tabnum{1.39} & \tabnum{0.01} & \tabnum{0.14} & \tabnum{1.39} \\
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{1.41} & \tabnum{5.54} & \tabnum{15.27} & \tabnum{1.70} & \tabnum{5.44} & \tabnum{15.94} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{2.21} & \tabnum{8.11} & \tabnum{23.30} & \tabnum{2.07} & \tabnum{7.95} & \tabnum{23.77} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{1.68} & \tabnum{8.11} & \tabnum{25.50} & \tabnum{1.46} & \tabnum{7.52} & \tabnum{24.04} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{2.76} & \tabnum{10.33} & \tabnum{31.23} & \tabnum{2.31} & \tabnum{9.21} & \tabnum{30.79} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{3.30} & \tabnum{12.03} & \tabnum{32.82} & \tabnum{3.55} & \tabnum{13.12} & \tabnum{35.70} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{3.92} & \tabnum{13.43} & \tabnum{35.25} & \tabnum{3.35} & \tabnum{12.48} & \tabnum{35.91} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{4.02} & \tabnum{13.50} & \tabnum{35.48} & \tabnum{3.97} & \tabnum{14.98} & \tabnum{37.63} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{4.26} & \tabnum{14.89} & \tabnum{37.30} & \tabnum{4.22} & \tabnum{14.64} & \tabnum{38.86} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{5.50} & \tabnum{19.25} & \tabnum{44.89} & \tabnum{5.97} & \tabnum{\underline{20.57}} & \tabnum{\underline{49.10}} \\
    \midrule
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$& \tabnum{\underline{7.31}} & \tabnum{\underline{21.29}} & \tabnum{\underline{45.26}} & \tabnum{\underline{6.65}} & \tabnum{\underline{20.57}} & \tabnum{45.85} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B)& \tabnum{\textbf{8.24}} & \tabnum{\textbf{24.54}} & \tabnum{\textbf{49.24}} & \tabnum{\textbf{8.56}} & \tabnum{\textbf{24.29}} & \tabnum{\textbf{50.70}} \\
    \bottomrule
  \end{tabularx}

\ifdefined\jointbootstrap\endgroup\else\end{table*}\fi


==> tables/zero_shot.tex <==
\ifdefined\jointmaintables\begingroup\else\begin{table*}[t]\fi
  \caption{\textbf{Model comparison on zero-shot classification across ten biomedical domains.} We report accuracy (\%) on 67 tasks from 43 datasets. We average tasks within each dataset, then datasets within each domain. `Overall' is the domain-balanced mean accuracy, with equal weight for each of the 10 domains.
  Cell: cellular phenotyping. Struct.: structure profiling. Micro.: microscopy composition. Histo.: histopathology. Radiol.: radiology. Ophth.: ophthalmology. Derm.: dermatology. Microb.: microbial and parasitic recognition. Surgery: surgery and anatomy. For \methodname{}, Scratch and DFN-2B denote random and DFN-2B initialization of the vision encoder, respectively; in both cases we use the same pretrained text encoder. $^{\ast}$ denotes random vision-encoder initialization for image-text pretraining. Among biomedical models, \textbf{bold} and \underline{underlined values} indicate the best and second-best scores in each column, respectively.}
  \vspace{-1mm}
  \label{tab:zero-shot}
  \centering
  \resulttablefont
  \renewcommand{\arraystretch}{1.05}
  \setlength{\tabcolsep}{0.8pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.17\textwidth}>{\centering\arraybackslash}p{0.065\textwidth}*{11}{Y}}
    \toprule
    \textbf{Model} & \textbf{Params.} & \multicolumn{1}{c}{\textbf{Cell}} & \multicolumn{1}{c}{\textbf{Struct.}} & \multicolumn{1}{c}{\textbf{Micro.}} & \multicolumn{1}{c}{\textbf{Cytology}} & \multicolumn{1}{c}{\textbf{Histo.}} & \multicolumn{1}{c}{\textbf{Radiol.}} & \multicolumn{1}{c}{\textbf{Ophth.}} & \multicolumn{1}{c}{\textbf{Derm.}} & \multicolumn{1}{c}{\textbf{Surgery}} & \multicolumn{1}{c}{\textbf{Microb.}} & \multicolumn{1}{c}{\textbf{Overall}} \\
    \midrule
    Random & - & \tabnum{18.65} & \tabnum{17.78} & \tabnum{34.42} & \tabnum{13.77} & \tabnum{28.96} & \tabnum{38.18} & \tabnum{29.67} & \tabnum{13.23} & \tabnum{19.63} & \tabnum{29.23} & \tabnum{24.35} \\
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext}  &  430M & \tabnum{22.18} & \tabnum{33.45} & \tabnum{56.86} & \tabnum{41.56} & \tabnum{39.80} & \tabnum{36.31} & \tabnum{50.53} & \tabnum{17.37} & \tabnum{23.05} & \tabnum{31.48} & \tabnum{35.26} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive}  &  428M & \tabnum{24.49} & \tabnum{44.44} & \tabnum{59.04} & \tabnum{10.25} & \tabnum{41.03} & \tabnum{64.86} & \tabnum{42.80} & \tabnum{15.67} & \tabnum{31.26} & \tabnum{44.87} & \tabnum{37.87} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining}  &  137M & \tabnum{28.16} & \tabnum{48.95} & \tabnum{69.20} & \tabnum{15.16} & \tabnum{57.30} & \tabnum{53.91} & \tabnum{38.74} & \tabnum{16.34} & \tabnum{29.09} & \tabnum{38.16} & \tabnum{39.50} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport}   &   800M & \tabnum{22.74} & \tabnum{44.77} & \tabnum{65.31} & \tabnum{37.28} & \tabnum{38.77} & \tabnum{49.26} & \tabnum{49.24} & \tabnum{20.62} & \tabnum{19.38} & \tabnum{\underline{58.58}} & \tabnum{40.59} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation}  &  196M & \tabnum{24.11} & \tabnum{49.59} & \tabnum{74.55} & \tabnum{11.16} & \tabnum{53.02} & \tabnum{55.36} & \tabnum{38.27} & \tabnum{30.48} & \tabnum{41.83} & \tabnum{43.63} & \tabnum{42.20} \\
    Panel2Patch~\cite{yuan2026panel2patch} & 428M & \tabnum{29.40} & \tabnum{47.12} & \tabnum{75.66} & \tabnum{9.50} & \tabnum{52.30} & \tabnum{\underline{63.31}} & \tabnum{47.56} & \tabnum{43.76} & \tabnum{37.34} & \tabnum{27.77} & \tabnum{43.37} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica}  &  428M & \tabnum{24.79} & \tabnum{56.53} & \tabnum{69.39} & \tabnum{8.97} & \tabnum{51.34} & \tabnum{60.85} & \tabnum{46.38} & \tabnum{43.76} & \tabnum{41.35} & \tabnum{32.25} & \tabnum{43.56} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong}  &  454M & \tabnum{25.62} & \tabnum{51.49} & \tabnum{76.23} & \tabnum{35.61} & \tabnum{53.94} & \tabnum{60.73} & \tabnum{35.53} & \tabnum{40.87} & \tabnum{37.38} & \tabnum{28.62} & \tabnum{44.60} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc}  &  428M & \tabnum{28.60} & \tabnum{\underline{57.60}} & \tabnum{66.17} & \tabnum{\underline{38.18}} & \tabnum{59.49} & \tabnum{55.57} & \tabnum{51.40} & \tabnum{\underline{45.49}} & \tabnum{35.11} & \tabnum{50.11} & \tabnum{48.77} \\
    \midrule
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$ & 454M & \tabnum{\textbf{34.22}} & \tabnum{56.69} & \tabnum{\textbf{79.70}} & \tabnum{37.96} & \tabnum{\underline{61.81}} & \tabnum{\textbf{64.57}} & \tabnum{\underline{56.65}} & \tabnum{38.75} & \tabnum{\underline{52.65}} & \tabnum{45.90} & \tabnum{\underline{52.89}} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B) & 454M & \tabnum{\underline{31.05}} & \tabnum{\textbf{59.73}} & \tabnum{\underline{76.32}} & \tabnum{\textbf{45.61}} & \tabnum{\textbf{62.55}} & \tabnum{61.40} & \tabnum{\textbf{61.64}} & \tabnum{\textbf{48.21}} & \tabnum{\textbf{57.62}} & \tabnum{\textbf{64.09}} & \tabnum{\textbf{56.82}} \\
    \bottomrule
  \end{tabularx}

\ifdefined\jointmaintables\endgroup\else\end{table*}\fi


==> tables/zero_shot_auc.tex <==
\ifdefined\jointauccap\begingroup\else\begin{table*}[t]\fi
  \caption{\textbf{One-vs-rest AUC across ten biomedical domains.} We report mean class AUC (\%) using the same prompts and aggregation as the main-paper accuracy results. Biomedical model rows are ordered by the corresponding Overall score from low to high. Abbreviations follow the main-paper accuracy table. $^{\ast}$ denotes random vision-encoder initialization for image-text pretraining. Among biomedical models, bold and underlined values indicate the best and second-best scores in each column, respectively.}
  \label{tab:zero-shot-auc}
  \centering
  \resulttablefont
  \ifdefined\jointauccap\renewcommand{\arraystretch}{1.0}\else\renewcommand{\arraystretch}{1.12}\fi
  \setlength{\tabcolsep}{1.4pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.20\textwidth}*{11}{Y}}
    \toprule
    \textbf{Model} & \multicolumn{1}{c}{\textbf{Cell}} & \multicolumn{1}{c}{\textbf{Struct.}} & \multicolumn{1}{c}{\textbf{Micro.}} & \multicolumn{1}{c}{\textbf{Cytology}} & \multicolumn{1}{c}{\textbf{Histo.}} & \multicolumn{1}{c}{\textbf{Radiol.}} & \multicolumn{1}{c}{\textbf{Ophth.}} & \multicolumn{1}{c}{\textbf{Derm.}} & \multicolumn{1}{c}{\textbf{Surgery}} & \multicolumn{1}{c}{\textbf{Microb.}} & \multicolumn{1}{c}{\textbf{Overall}} \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{57.40} & \tabnum{71.24} & \tabnum{82.57} & \tabnum{64.76} & \tabnum{69.28} & \tabnum{48.67} & \tabnum{55.37} & \tabnum{62.17} & \tabnum{57.75} & \tabnum{57.82} & \tabnum{62.70} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{62.83} & \tabnum{77.18} & \tabnum{87.32} & \tabnum{58.69} & \tabnum{74.56} & \tabnum{53.15} & \tabnum{52.15} & \tabnum{63.24} & \tabnum{60.73} & \tabnum{66.73} & \tabnum{65.66} \\
    \midrule
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{70.36} & \tabnum{80.15} & \tabnum{86.59} & \tabnum{56.60} & \tabnum{82.30} & \tabnum{68.52} & \tabnum{67.28} & \tabnum{63.15} & \tabnum{69.53} & \tabnum{60.74} & \tabnum{70.52} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{63.83} & \tabnum{82.15} & \tabnum{88.15} & \tabnum{59.18} & \tabnum{79.35} & \tabnum{71.18} & \tabnum{67.57} & \tabnum{71.03} & \tabnum{73.93} & \tabnum{65.77} & \tabnum{72.22} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{62.51} & \tabnum{79.14} & \tabnum{89.73} & \tabnum{55.66} & \tabnum{80.13} & \tabnum{74.36} & \tabnum{70.65} & \tabnum{65.27} & \tabnum{77.11} & \tabnum{68.95} & \tabnum{72.35} \\
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{71.61} & \tabnum{79.33} & \tabnum{91.33} & \tabnum{58.40} & \tabnum{79.66} & \tabnum{69.94} & \tabnum{68.32} & \tabnum{71.35} & \tabnum{74.22} & \tabnum{67.50} & \tabnum{73.16} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{61.90} & \tabnum{75.98} & \tabnum{85.64} & \tabnum{75.27} & \tabnum{71.97} & \tabnum{76.00} & \tabnum{75.75} & \tabnum{72.88} & \tabnum{68.08} & \tabnum{\underline{80.26}} & \tabnum{74.37} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{66.42} & \tabnum{82.51} & \tabnum{90.72} & \tabnum{69.79} & \tabnum{81.97} & \tabnum{77.36} & \tabnum{72.82} & \tabnum{74.52} & \tabnum{81.65} & \tabnum{74.21} & \tabnum{77.20} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{72.33} & \tabnum{\textbf{86.36}} & \tabnum{\underline{92.46}} & \tabnum{76.47} & \tabnum{\underline{85.34}} & \tabnum{77.74} & \tabnum{77.55} & \tabnum{76.51} & \tabnum{79.53} & \tabnum{79.57} & \tabnum{80.39} \\
    \midrule
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$ & \tabnum{\textbf{73.59}} & \tabnum{82.69} & \tabnum{\textbf{93.83}} & \tabnum{\underline{80.75}} & \tabnum{85.02} & \tabnum{\textbf{78.76}} & \tabnum{\textbf{80.39}} & \tabnum{\underline{78.66}} & \tabnum{\underline{82.65}} & \tabnum{\textbf{83.79}} & \tabnum{\underline{82.01}} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B) & \tabnum{\underline{73.01}} & \tabnum{\underline{84.74}} & \tabnum{91.94} & \tabnum{\textbf{83.44}} & \tabnum{\textbf{86.71}} & \tabnum{\underline{78.09}} & \tabnum{\underline{80.00}} & \tabnum{\textbf{81.24}} & \tabnum{\textbf{85.58}} & \tabnum{79.16} & \tabnum{\textbf{82.39}} \\
    \bottomrule
  \end{tabularx}

\ifdefined\jointauccap\endgroup\else\end{table*}\fi


==> tables/zero_shot_f1.tex <==
\ifdefined\jointauccap\begingroup\else\begin{table*}[t]\fi
  \caption{\textbf{Macro-F1 across ten biomedical domains.} We report strict class Macro-F1 (\%) using the same prompts and aggregation as the main-paper accuracy results. Biomedical model rows are ordered by the corresponding Overall score from low to high. Abbreviations follow the main-paper accuracy table. $^{\ast}$ denotes random vision-encoder initialization for image-text pretraining. Among biomedical models, bold and underlined values indicate the best and second-best scores in each column, respectively.}
  \label{tab:zero-shot-f1}
  \centering
  \resulttablefont
  \ifdefined\jointauccap\renewcommand{\arraystretch}{1.0}\else\renewcommand{\arraystretch}{1.12}\fi
  \setlength{\tabcolsep}{1.4pt}
  \begin{tabularx}{\textwidth}{>{\raggedright\arraybackslash}p{0.20\textwidth}*{11}{Y}}
    \toprule
    \textbf{Model} & \multicolumn{1}{c}{\textbf{Cell}} & \multicolumn{1}{c}{\textbf{Struct.}} & \multicolumn{1}{c}{\textbf{Micro.}} & \multicolumn{1}{c}{\textbf{Cytology}} & \multicolumn{1}{c}{\textbf{Histo.}} & \multicolumn{1}{c}{\textbf{Radiol.}} & \multicolumn{1}{c}{\textbf{Ophth.}} & \multicolumn{1}{c}{\textbf{Derm.}} & \multicolumn{1}{c}{\textbf{Surgery}} & \multicolumn{1}{c}{\textbf{Microb.}} & \multicolumn{1}{c}{\textbf{Overall}} \\
    \midrule
    CoCa$^{\ast}$~\cite{yu2022cocacontrastivecaptionersimagetext} & \tabnum{14.77} & \tabnum{22.40} & \tabnum{35.10} & \tabnum{15.04} & \tabnum{29.59} & \tabnum{17.58} & \tabnum{25.29} & \tabnum{13.04} & \tabnum{14.39} & \tabnum{21.12} & \tabnum{20.83} \\
    OpenCLIP$^{\ast}$~\cite{cherti2023reproduciblescalinglawscontrastive} & \tabnum{17.25} & \tabnum{34.54} & \tabnum{31.19} & \tabnum{6.37} & \tabnum{32.25} & \tabnum{29.36} & \tabnum{25.11} & \tabnum{11.92} & \tabnum{16.69} & \tabnum{32.12} & \tabnum{23.68} \\
    \midrule
    Panel2Patch~\cite{yuan2026panel2patch} & \tabnum{19.94} & \tabnum{38.18} & \tabnum{62.93} & \tabnum{5.85} & \tabnum{44.05} & \tabnum{38.31} & \tabnum{24.76} & \tabnum{13.64} & \tabnum{25.20} & \tabnum{21.27} & \tabnum{29.41} \\
    \mbox{BMC-CLIP-CF}~\cite{lozano2025biomedica} & \tabnum{14.58} & \tabnum{44.27} & \tabnum{57.25} & \tabnum{6.23} & \tabnum{42.43} & \tabnum{38.46} & \tabnum{24.72} & \tabnum{15.23} & \tabnum{26.26} & \tabnum{25.84} & \tabnum{29.53} \\
    \mbox{PMC-CLIP}$^{\ast}$~\cite{lin2023pmcclipcontrastivelanguageimagepretraining} & \tabnum{20.64} & \tabnum{36.74} & \tabnum{59.29} & \tabnum{7.33} & \tabnum{44.07} & \tabnum{37.91} & \tabnum{28.07} & \tabnum{13.03} & \tabnum{21.68} & \tabnum{27.49} & \tabnum{29.62} \\
    MedSigLIP~\cite{sellergren2025medgemmatechnicalreport} & \tabnum{15.36} & \tabnum{30.03} & \tabnum{57.37} & \tabnum{19.74} & \tabnum{31.45} & \tabnum{39.63} & \tabnum{36.83} & \tabnum{16.53} & \tabnum{14.13} & \tabnum{36.09} & \tabnum{29.71} \\
    BiomedCLIP~\cite{zhang2023biomedclipmultimodalbiomedicalfoundation} & \tabnum{17.62} & \tabnum{34.31} & \tabnum{61.83} & \tabnum{6.10} & \tabnum{42.35} & \tabnum{41.01} & \tabnum{31.85} & \tabnum{14.97} & \tabnum{29.13} & \tabnum{28.30} & \tabnum{30.75} \\
    \mbox{BMC-LongCLIP}~\cite{sun2025tokenswastedleveraginglong} & \tabnum{17.39} & \tabnum{40.00} & \tabnum{63.86} & \tabnum{16.65} & \tabnum{39.59} & \tabnum{45.48} & \tabnum{30.91} & \tabnum{19.83} & \tabnum{28.32} & \tabnum{25.00} & \tabnum{32.70} \\
    \mbox{MedPMC-CLIP}~\cite{kim2026medpmc} & \tabnum{21.74} & \tabnum{\underline{52.67}} & \tabnum{44.09} & \tabnum{24.96} & \tabnum{\underline{50.49}} & \tabnum{43.53} & \tabnum{40.80} & \tabnum{23.74} & \tabnum{23.49} & \tabnum{33.31} & \tabnum{35.88} \\
    \midrule
    \rowcolor{bioloomlight}
    \methodname{} (Scratch)$^{\ast}$ & \tabnum{\textbf{25.49}} & \tabnum{43.90} & \tabnum{\textbf{66.09}} & \tabnum{\underline{27.30}} & \tabnum{48.91} & \tabnum{\textbf{48.76}} & \tabnum{\underline{45.05}} & \tabnum{\underline{27.11}} & \tabnum{\underline{38.23}} & \tabnum{\underline{38.13}} & \tabnum{\underline{40.90}} \\
    \rowcolor{bioloomlight}
    \methodname{} (DFN-2B) & \tabnum{\underline{22.40}} & \tabnum{\textbf{53.68}} & \tabnum{\underline{64.92}} & \tabnum{\textbf{32.45}} & \tabnum{\textbf{52.77}} & \tabnum{\underline{47.97}} & \tabnum{\textbf{50.43}} & \tabnum{\textbf{31.41}} & \tabnum{\textbf{41.20}} & \tabnum{\textbf{39.90}} & \tabnum{\textbf{43.71}} \\
    \bottomrule
  \end{tabularx}

\ifdefined\jointauccap\endgroup\else\end{table*}\fi

